Optimal Energy Consumption with Communication, Computation, Caching and QoI-Guarantee

Energy efficiency is a fundamental requirement of modern data communication systems, and its importance is reflected in much recent work on performance analysis of system energy consumption. However, most works have only focused on communication and computation costs, but do not account for caching costs. Given the increasing interest in cache networks, this is a serious deficiency. {In this paper, we consider the problem of energy consumption in data communication, compression and caching (C$3$) with a Quality of Information (QoI) guarantee in a communication network. {Our goal is to identify the optimal data compression rate and data placement over the network to minimize the overall energy consumption in the network.} he formulated problem is a \emph{Mixed Integer Non-Linear Programming} (MINLP) problem with non-convex functions, which is NP-hard in general. } {We} propose a variant of spatial branch and bound algorithm (V-SBB), that can {provide} the $\epsilon$-global optimal solution to {our problem}. {We numerically show that our C3 optimization framework can improve the energy efficiency up to 88\% compared to any C2 optimization between communication and computation or caching. Furthermore, for our energy consumption problem, V-SBB {provides comparatively better solution than some other MINLP solvers.}}

==> 01-intro.tex <==


%\red{Large volume of data has been generated over the last couple of years by a large number of different Information and Communication Technology (ICT) devices. These data need to be efficiently compressed, transmitted, and cached to satisfy the Quality of Information (QoI) required by end users or applications such as data analytics \cite{heintz16}. While ICT devices are primarily intended to improve the services provided to the users by providing better connectivity,  two basic challenges that have arisen as a result of the increase in number of devices (and consequently the amount of data) are 1)  higher operational energy costs of the ICT networks 2) inability to transmit such enormous data through traditional networks due to limited bandwidth.}% 3) geographic distribution of the data producing nodes.}

Large quantities of data are generated continuously over time in the form of sensor reading, posts, emails etc.  {An efficient} communication {and processing} system must provide efficient data analytics \cite{heintz16,heintz15} to extract useful and timely information for the user.  Hence, there is a growing interest in designing distributed data analytics platforms \cite{boykin14}.

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{distributed-model.pdf}
	\caption{The distributed model for a typical data analytics service consists of a single central and multiple edge servers in a hub-and-spoke architecture.}
	\label{fig:distributed-model}
	\vspace{-0.25in}
\end{figure} 

In many data analytics systems, data is often generated and gathered from sources such as mobile devices, users and sensors at {dispersed locations}.  As a result, the distributed infrastructure of a typical data analytics service (e.g., Google Analytics, Amazon Web Services etc) has a \emph{hub-and-spoke} model (see Figure~\ref{fig:distributed-model}).  Data are generated and sent to ``edge" servers\footnote{{In this paper, we interchange the notion of (center and edge) server and node.}} near them.  The edge servers are usually geographically distributed and process (e.g. {compress}) the incoming data and send {the resultant data} to other servers {for} further process{ing} and {storage}.


While each server is able to process and store data, {its} resources are typically limited. In particular, the storage capacity and available power for data compression m{ay} be limited. It has been reported that  the average annual power consumption for data analytics was $25$ Giga-Watts in $2013$ \cite{klein2016ict,energy}, which is equivalent to operating $23$ nuclear reactors.  This not only increases the operational costs but also has an adverse {environmental impact}.  Energy consumption is also a fundamental challenge for many wireless components that operate on limited battery power supply and are usually deployed in remote or inaccessible areas.    Furthermore, about $5$ zetta-bytes of data pass through the global network in $2017$ \cite{belllabs}. This not only requires {a huge} network bandwidth, but may further increase the energy expenditure as communicating such {a} large amount of data in  a distributed environment incurs {tremendous} transmission costs. These challenges necessitate the need for designs that can enhance the  energy efficiency of distributed system with a QoI guarantee.   


Typically there are two approaches {to} data analytics.  On one hand,  a \emph{centralized approach} {can be} applied where all the {collected} data is sent to the centralized server and no processing is performed at the edge {or intermediate nodes}.  However, such a centralized approach is often suboptimal {and even infeasible}, since it may cause large delay due to the limited {communication} bandwidth  and does not make use of the available computation and storage resources at edges.   On the other hand, a \emph{decentralized approach} utilizes the edge resources to compute and store the data to reduce the network traffic.   In this paper, we argue that data analytics must utilize both edges and center resources in a well-organized coordinated manner so as to achieve the minimal energy consumption {by proper tradeoffs among} data communication, computation and caching {while satisfying}  stringent {quality-of-information} (QoI) requirements {of the} end users.
%\red{  The average annual ICT power consumption was 122 Giga-Watts (GW) in 2013 \cite{klein2016ict} that is equivalent to operating 117 nuclear reactors. This not only increases the operational costs but can have adverse affects on the environment. Energy consumption is also a fundamental challenge for many wireless components that operate on limited battery power supply and are usually deployed in remote or inaccessible areas.    Furthermore, about five zetta-bytes (ZB) of data has passed through the global network in 2017 \cite{belllabs}. This not only requires higher network bandwidth, but may further increase the energy expenditure as communicating such large amount of data in  a distributed environment incurs higher transmission costs. These challenges necessitate the need for  designs that can enhance the  energy efficiency of a distributed system with a QoI guarantee.   } 



Data computation has been widely used in data analytics systems.  It combines and compresses large quantities of {generated data from data generators that} must be processed in a specified time period. For example, Google Analytics can compute the total visits to one website from different regions and aggregate the visitors' information on an hourly basis.  Data {compression (computation) can lower} transmission cost by {removing} the inherent redundancy in the data and reducing the total amount of data {for further transmission}  at the expense of computational cost. 


Furthermore, cache has become an {important} component of  data analytics systems to store information locally.  For instance, {users in a geographical area want} to receive the same information (e.g., live videos, commentary) generated by a number of data sources.  In such cases, caching can be used as a mean to reduce the access latency (resulting in enhanced QoI) by storing the data generated in a finite period {at some locations} to serve {the users}.  This can also help reduce the energy cost and bandwidth consumption as data are stored closer to the requesting nodes, eliminating the need for {repeated} transmissions from the source nodes that may be far away {from the requesting users}.  {For example, caches have been widely used in wireless sensor networks (WSNs) and its functionality in minimizing latency and reducing energy cost has been studied in \cite{dimokas2008cooperative,dimokas2011high,alipio2017cache}. } However, data caching also consumes energy \cite{li2013energy}.


%\red{\emph{Data compression} and \emph{data caching} may reduce the energy consumption in any distributed system. Compression reduces transmission (communication) cost by exploiting the inherent redundancy in the data and reducing the total amount of data transmitted  at the expense of computational cost.  Similarly, while caching is primarily intended to reduce the access latency (resulting in enhanced QoI), it can also help reduce the energy cost and bandwidth consumption as data is stored closer to the requesting nodes, eliminating the need for  multiple retransmissions from the source nodes that may be far away. However, data caching also consumes energy \cite{li2013energy}.  Hence there exists a trade-off among data communication, computation (compression) and caching energy costs.  }

{Due to the inter-dependence}, there exists a tradeoff among data communication, computation and caching energy costs.  In this paper, we formulate an optimization problem that characterizes the tradeoff among communication, computation, and caching energy cost with QoI guarantee, {and then develop an efficient algorithm to solve the optimization problem}.   {\emph{Our algorithm {decides} how much  data compression should be performed at each node and where data {should} be cached in the system.}} {Without loss of generality (W.l.o.g.),} each node {is assumed to have} ability to compress and cache data {up to} some finite storage capacity.
%\end{comment}

%The rapid growth of smart environments, and advent of Internet of Things (IoT) have led to the generation of large amounts of data. However, it is a daunting task to transmit enormous data through traditional networks due to limited bandwidth and energy limitations  \cite{nazemi2016qoi}. 
%These data need to be efficiently compressed, transmitted, and cached to satisfy the Quality of Information (QoI) required by end users.  In fact, 

%A particular example of modern systems that require high energy efficiency is the wireless sensor network (WSN). Consider a WSN with various types of sensors, which can generate enormous amount of data to serve  end users.  On one hand, data compression has been adopted to reduce transmission (communication) cost at the expense of computation cost.  On the other hand, caches can be used as a mean of reducing transmission costs and access latency, thus  enhancing QoI but with the expense of the added caching cost.  Hence, there exists a tradeoff in energy consumption due to  data communication, computation and caching.  This raises the question: what is the right balance between compression and caching so as to minimize the total energy consumption of the network?


\subsection{Motivation}
The setting of interest in this paper {consists} of a large number of (edge and center) servers, each equipped with finite storage capacity and data computation capability.  Examples of such settings are WSNs, smart {cities} or Internet of Things (IoTs) where geographically distributed servers generate a large amount of data.  In this paper, we focus on WSNs, particularly in the context of tactical environments \cite{elmasry2010comparative} as {an illustrative example}.   Wireless sensors are significant components in tactical environments which have limited bandwidth, energy resources but stringent requirements (e.g., low latency). %\red{ Tactical networks \cite{elmasry2010comparative}  primarily consist of wireless sensors that are optimized for use in military environments. Tactical networks have limited bandwidth, limited energy resources, and stringent requirements (such as low access latency, high security).} 
In WSNs, sensors generate, process and transmit data to nearby edge servers, which can further process the data.  {As shown in}  Figure~\ref{fig:distributed-model}, we consider a tree-structured {geo-distributed} WSN.  All sensors are battery operated and {thus have limited power supply}.  {W.l.o.g, data is generated only by the leaf nodes (sensors) and the goal of the network is to process the generated data while it is being forwarded toward the sink (root) node. The network also contains relay nodes that do not produce their own data, but can compress and cache data received from their corresponding children nodes.}
%Therefore, {the network contains} relay nodes that do not produce their own data, but can compress and cache  data generated by leaf nodes (sensors).   In particular, %as shown in Figure~\ref{fig:example}, 
%we assume that only edge sensors generate data, and there exists a 
{The} sink node {also receives}  and serves the requests for the data generated in this network.  The relay nodes allow the leaf nodes to transmit over shorter range, hence reducing the energy consumption of the leaf nodes. Furthermore, the wireless channel conditions may also not be suitable for long range communications. The relay nodes transmit the data up the tree until it reaches the root node that satisfies any requests for the data of any particular leaf node.  {To continue, let us describe several key terms as follows.}

%The requests for the data can be from different users who are interested in the activity in a geographic location.  Below we describe some key terms. % \red{\bf [comment: Do you think it would be better to give an example of such a wireless sensor network? Like the seismic sensors earlier, or in fact we can even give an example of IoT sensors. The reviewer might hit us again with the comment that this is not usually the case. We have built the story now along the lines of geo-distributed systems but still it might be better to given an example.]} \blue{\bf[Will edit something here later.]}



% \red{There are different motivating examples for our work  such as wireless sensor network (WSN), smart home/cities sensor data, Internet of Things (IoT) or the sensor data produced at different geographically dispersed nodes. In such networks, sensors transmit their data to nearby ``edge'' servers or other nodes that apply some computation procedure on the data and  forwards the data to node up in the hierarchy and finally a central entity which we call the ``root'' node. This can be modeled as a tree-structured network where the leaf nodes are the sensors, the edge servers or other nodes are the intermediate nodes while the central processing entity is root node. We primarily focus on a WSN scenario. Consider a geographically distributed network of seismic sensors that sense the seismic activity as shown in Figure \blue{\bf [comment: add the Figure]}. These sensors are battery operated and inaccessible for battery replacement. Therefore, relay nodes that do not produce their own data, but can compress and cache the data of leaf nodes/sensors are used. The relay nodes allow the leaf nodes to transmit over shorter range, hence reducing the energy consumption of the leaf nodes. Furthermore, the wireless channel conditions may also not be suitable for long range communications. The relay nodes transmit the data up in the tree until it reaches the root node that satisfies any requests for the data of any particular sensor leaf node. The requests for the data can be from different users around the globe who are interested in the seismic activity in a geographic location. Below we describe some key terms.   }


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{figures/wsn-new.pdf}
%\caption{A general wireless sensor network.}
%\label{fig:example}
%\vspace{-0.2in}
%\end{figure} 


\noindent{\textit{Computation:}} 
Data aggregation \cite{rajagopalan06, fasolo07} is the process of gathering data from multiple generators (e.g., sensors), compressing them to eliminate redundant information and then  providing the summarized  information to end users.  Since only part of the original data is transmitted, data aggregation can conserve a large amount of energy.  A common assumption in previous work is that {the amount of} energy {consumed by data compression} is smaller than that needed to transmit {the same amount of} data.  {Therefore, data compression was considered a viable technique for reducing energy consumption. } %Therefore,  %\red{data compression would always reduce the net-energy consumption in the network. }
%there exists a benefit for data compression by neglecting the computational energy cost. 
However, it has been shown \cite{barr2006energy} that computational energy cost can be significant and may cause a net-energy increase if  data are compressed beyond a certain  {level (threshold)}. Hence, it is necessary to {jointly} consider both  transmission and computation costs, and it is important to characterize the tradeoff between them \cite{nazemi2016qoi}.


\noindent{\textit{Caching:}} \emph{Cache has} been widely used in networks and distributed systems to improve performance by storing information locally, which jointly reduces access latency and bandwidth requirements, and hence improves user experience.  %\red{Content Distribution Networks (CDNs), Software Defined Networks (SDNs),  Named Data Networks (NDNs) and Content Centric Networks (CCNs) are important examples of such systems.}  
The {basic} idea behind caching is to make information available at a location closer to the user.  Again, most  previous work focused on designing caching algorithms to enhance system performance without considering the energy cost of caching.  However, caching itself can incur significant energy costs \cite{choi2012network}.  Therefore, capturing caching cost and characterizing the tradeoff between communication and caching energy cost are also critical for system design.  



\noindent{\textit{Quality of Information (QoI):}} The notion of QoI required by end users is affected by many factors. In particular, the degree of the data aggregation in a system is crucial for QoI.  %\cite{ehikioya1999characterization} studied the impact of data aggregation on end user QoI and showed that it can deteriorate QoI in some situations. 
It has been shown that data aggregation can deteriorate QoI in some situations \cite{ehikioya1999characterization}. 
Thus an energy efficient design for appropriate data aggregation with a guaranteed QoI is desirable. 



%We focus on a tree-structured sensor network where each leaf node generates  data, and compresses and transmits the data to the sink node in the network, which serves the requests for these data from devices outside this network.  Examples of such a setting are military sites, wireless sensors or societal networks, where a large number of devices gather data, and desire to transmit the local information to any device outside this network that requires this information.  

The objective of this work is to develop an efficient algorithm to minimize the total energy cost by incorporating data communication, computation and caching energy costs with a desired QoI constraint into our {formulation}, so that {the} optimal data compression rate at each node and {the} optimal {data} caching location in the network can be determined.  Such an algorithm should be lightweight and achieve {the} optimal solution efficiently.  



\subsection{Organization and Main Results}
In Section~\ref{sec:model}, we describe our system model in which nodes are logically arranged as a tree. Each node receives and compresses data from its children node(s). The compressed data are transmitted and further compressed {by upstream nodes} towards the sink node.  Each node can also cache the compressed data locally.  In Section~\ref{sec:opt}, we formulate the problem of energy-efficient data compression, communication and caching with QoI constraint as a non-convex mixed integer non-linear programming (MINLP) problem, which is hard to solve in general. We then show that there exists an equivalent problem obtained through symbolic reformation \cite{smith1996global} in Section~\ref{sec:sBNB}, and propose a variant of the Spatial Branch-and-Bound (V-SBB) algorithm to solve it.  {We show that our proposed algorithm can achieve  $\epsilon$-global optimality of the original MINLP efficiently.  Since we have a discrete space and a non-convex problem, showing that there exists an $\epsilon$-optimal solution  and developing an efficient algorithm to achieve it are quite intricate.  This is another contribution in this paper.}


In Section~\ref{sec:results}, we evaluate the performance of our optimization framework and the proposed V-SBB algorithm  through extensive numerical studies.  In particular, we make a thorough comparison with other MINLP solvers Bonmin \cite{bonami2008algorithmic}, NOMAD \cite{le2011algorithm},  and Matlab's genetic algorithm (GA) under different network scenarios.  The results show that our algorithm can achieve {the} $\epsilon$-global optimality,  and is either comparable to or outperforms Bonmin.  Furthermore, our algorithm is more robust and stable in the context of varying network situations. In other words, Bonmin in certain cases is not able to provide a solution, even though  the original problem is feasible.  Furthermore, our algorithm  easily outperforms NOMAD and Matlab's GA \cite{deb2002fast} in most of {our testing} scenarios.  More importantly, we observe that with the joint optimization of data communication, computation and caching (C$3$),  energy efficiency can be improved by as much as $88\%$ compared to only optimizing communication and computation, or communication and caching (C$2$).  This further strengthens the contributions of our optimization framework {of C$3$}.   {In Section~\ref{sec:relatedwork}, we review previous work,  and conclude in Section~\ref{sec:con}.}








==> 02-related.tex <==


While optimizing energy costs in wireless sensor networks has been extensively studied \cite{heinzelman2000energy,ye2002energy}, existing work primarily is concerned with routing \cite{manjeshwar2001teen}, MAC protocols \cite{heinzelman2000energy}, and clustering \cite{ye2005eecs}. With the growing deployment of smart sensors in modern systems \cite{nazemi2016qoi}, in-network data processing, such as data aggregation, has been widely used as a mean of reducing system energy cost by lowering the data volume for transmission. 

%Optimizing the energy consumption of wireless sensors has been extensively studied in literature \cite{heinzelman2000energy,ye2002energy} as energy is one of the fundamental limitations of battery operated devices. Initial work was primarily concerned with routing (such as \cite{manjeshwar2001teen}) and MAC \cite{heinzelman2000energy} protocols as well as clustering \cite{ye2005eecs} with the overall objective of minimizing communication energy and extending the lifetime of the sensor network.  However, with the advent of smart sensors and the presence of temporal and spatial relationship among the data generated by the sensors, in-network data processing (such as data fusion/aggregation or compression) emerged as a method to reduce the overall communication energy costs by reducing the total number of bits that were transmitted. However, Barr et al. \cite{barr2006energy} showed that  data compression beyond a certain threshold can consume more energy than communication energy. 


\noindent{\textit{Communication and Computation Energy Costs:} 
%Therefore, recent works such as \cite{nazemi2016qoi,laporta2012,anandkumar2009energy,zhang2006distributed,yu2008data} have considered both communication and in-network processing costs to  minimize the overall energy consumption in the sensor network.
Energy efficient inference in a random fusion network without QoI guarantee was considered in \cite{anandkumar2009energy}.  Network Utility Maximization (NUM) framework was applied in \cite{laporta2012} to obtain optimal compression rate for data aggregation as well as optimal locations for performing data compression.   The optimal energy allocation between communication and sensing to maximize the total information received at the sink node was studied in \cite{zhang2006distributed}, but they did not consider data computation.  An efficient algorithm for data compression in a  data gathering tree was proposed in \cite{yu2008data}.  \cite{nazemi2016qoi} presented a distributed algorithm to minimize overall energy costs in a tree structured network by optimizing the compression factor at  each node. 

None of these works considered caching costs.  Since caches are already integral components of many modern systems, including wireless sensor networks, they can be used to improve performance by making data available at locations closer to end users %\red{which among many other advantages will also  
 to reduce the communication cost \cite{choi2012network}.


% Anandkumar et al. \cite{anandkumar2009energy} use a stochastic approach for modeling an energy- efficient distributed inference in any random fusion network. Their inference policy requires a centralized information center and they do not take QoI into consideration. Eswaran et al. \cite{laporta2012} utilize Network Utility Maximization (NUM) framework for obtaining the optimal compression and fusion rates for aggregating the data along with the optimal locations  for data processing using a convex  optimization framework. Zhang et al. \cite{zhang2006distributed} present a distributed algorithm for optimally allocating energy between communication and sensing at every single node for maximizing the total information received at the data sinks present in the network. Their work does not consider in-network processing. Yu et al. \cite{yu2008data} present an algorithm to create a data gathering tree that adopts a tunable data compression for overall energy efficiency in the network.  Nazemi et al. \cite{nazemi2016qoi} present a distributed algorithm that minimizes the overall energy consumption in a tree structured network by optimizing the compression factor for a trade-off between communication and computation energy. 

To the best of our knowledge, there is no prior work that jointly considers communication, computation and caching costs in data communication networks. One of the important contributions of this paper is to develop an optimization algorithm that minimizes the total system energy costs by characterizing the tradeoff between communication, computation and caching costs with a QoI guarantee for end users. %Here, we make a comparison between our work and previous results with respect to communication cost (Comm.C.), computation cost (Comp.C.), caching cost (Ca.C.) and QoI, as shown in Table \ref{tab:litcomparison}.   %\red{\bf It seems like we have never discussed and mentioned INP.}
%\blue{\bf[comment: I think the table should stay. Let's keep it for now]}
%The existing work does not take storage/caching into account for minimizing overall energy.  However, recent advances in sensor technology has allowed sensors to have memory for caching that can reduce the communication cost by locally storing a copy of data, eliminating the need for multiple transmissions from the source node \cite{choi2012network}. While NDN literature utilizes caching for enhancing the overall quality of service by minimizing latency as well as reducing the energy consumption by eliminating the need for multiple retransmissions from the source node, there is no existing work (to the best of our knowledge) that jointly considers communication, computation and caching cost to minimize overall energy consumption in the network subject to QoI constraints. In this work, we utilize a non-convex MINLP optimization framework to obtain the optimal compression ratio at every node for fundamental trade-off between data communication and compression. Furthermore, we leverage the presence of memory in sensors for data caching which  also reduces the net-energy consumption in network. Table \ref{tab:litcomparison} compares our work to some of the existing work, where TC, CC and CaC stand for transmission, computation and caching cost, respectively. 

%\begin{table}[ht]
%\vspace{-0.15in}
%	\centering
%	\caption{Comparison of related work with Ours}
%	\vspace{-0.1in}
%	\begin{tabular}{|c|c|c|c|c|}
%		\hline
%		\textbf{Related Work} & \textbf{Comm.C.} & \textbf{Comp.C.} & \textbf{Ca.C.} &  \textbf{QoI} \\ \hline
%	\cite{nazemi2016qoi}	&   $\checkmark$           &   $\checkmark$           &    $\times$                   &   $\checkmark$            \\ \hline
%	\cite{laporta2012}	&   $\checkmark$           &   $\checkmark$           &    $\times$                  &   $\checkmark$            \\ \hline
%		\cite{anandkumar2009energy}	&    $\checkmark$       &  $\checkmark$          &    $\times$                  &       $\times$         \\ \hline
%	\cite{zhang2006distributed}	&   $\checkmark$           &   $\checkmark$           &    $\times$                     &    $\times$           \\ \hline
%	\cite{yu2008data}	&   $\checkmark$           &   $\checkmark$           &    $\times$                       &    $\times$           \\ \hline
%	Ours 	&   $\checkmark$           &   $\checkmark$           &    $\checkmark$                     &    $\checkmark$           \\ \hline
%	\end{tabular}
%	\label{tab:litcomparison}
%\vspace{-0.15in}	
%\end{table}


%\begin{table}[ht]
%\vspace{-0.2in}
%	\centering
%	\caption{Comparison of related work with Ours}
%	\vspace{-0.1in}
%	\begin{tabular}{|c|c|c|c|c|c|}
%		\hline
%		\textbf{Related Work} & \textbf{Comm.C.} & \textbf{Comp.C.} & \textbf{Ca.C.} & \textbf{INP} & \textbf{QoI} \\ \hline
%	\cite{nazemi2016qoi}	&   $\checkmark$           &   $\checkmark$           &    $\times$          &      $\checkmark$         &   $\checkmark$            \\ \hline
%	\cite{laporta2012}	&   $\checkmark$           &   $\checkmark$           &    $\times$          &      $\checkmark$         &   $\checkmark$            \\ \hline
%		\cite{anandkumar2009energy}	&    $\checkmark$       &  $\checkmark$          &    $\times$          &   $\checkmark$         &       $\times$         \\ \hline
%	\cite{zhang2006distributed}	&   $\checkmark$           &   $\checkmark$           &    $\times$          &       $\times$        &    $\times$           \\ \hline
%	\cite{yu2008data}	&   $\checkmark$           &   $\checkmark$           &    $\times$          &        $\checkmark$       &    $\times$           \\ \hline
%	Ours 	&   $\checkmark$           &   $\checkmark$           &    $\checkmark$          &        $\checkmark$       &    $\checkmark$           \\ \hline
%	\end{tabular}
%	\label{tab:litcomparison}
%\end{table}
%







==> 03-model.tex <==
 


We represent the network as a directed graph $G=(V, E).$ %For simplicity \red{\bf [comment:  I think rather than using the word simplicity, we can say that since our example case or task at hand i.e., distributed analytics usually happens in a tree-structured network so we focus on that? ]}, 
As shown in Section~\ref{sec:intro}, a hub-and-spoke model shown in Figure~\ref{fig:distributed-model} usually exists in data analytics systems including WSNs.  W.l.o.g., we consider a tree, with $N=|V|$ nodes, as shown in Figure~\ref{fig:1}. Node $v \in V$ is capable of storing $S_v$ amount of data.  Let $\mathcal{K}\subseteq V$ with $K=|\mathcal{K}|$ be the set of leaf nodes, with $\mathcal{K}=\{1, 2, \cdots, K\}$.  Time is partitioned in periods of equal length $T>0$ and data generated in each period are independent, i.e., the transmitted and cached data in one time period may be totally replaced with new data for the next time period\footnote{In some literature, this is called \emph{windowed grouped data aggregation} where data generated in a finite time period must be compressed.}. %. Furthermore, we assume that the data in one time period do not change.}    
W.l.o.g., we consider one particular period in the remainder of the paper.  % \red{We assume that during a period ``T", the sensor data and cached data copy does not change. At time 'T+1', new sensor data is generated resulting in the old cached data being replaced with new data}. 
As is the case in a typical geo-distributed analytics system, we assume that only leaf nodes $k\in\mathcal{K}$ can generate data, and all other nodes in the tree receive and compress data from their children nodes, and either cache or transmit the compressed data to their parent nodes during time $T$.  Relaxation of the preceding assumptions is discussed in Section~\ref{sec:relaxation}. 

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{tree-network-new.pdf}
	\caption{Tree-Structured Network Model.}
	\protect\label{fig:1}
	\vspace{-0.3in}
\end{figure}


Let $y_k$ be the amount of data generated by leaf node $k\in\mathcal{K}$. The data generated at the leaf nodes are transmitted up the tree to the sink node $s,$ which serves the requests for the data generated in the network.  Let $h(k)$ be the depth of node $k$ in the tree. W.l.o.g., we assume that the sink node is located at level $h(s)=0.$  We represent the unique path from node $k$  to the sink node by $\mathcal{H}^k$ of length $h(k)$ the sequence $\{h_0^k, h_1^k, \cdots, h_{h(k)}^k\}$ of nodes $h_j^k\in V$ such that $(h_j^k, h_{j+1}^k)\in E,$ where $h_0^k\triangleq s$ (i.e., the sink node) and $h_{h(k)}^k\triangleq k$ (i.e., the node itself).  


We denote the per-bit reception, transmission and compression cost of node $v \in V$ as $\varepsilon_{vR}, \varepsilon_{vT}$, and $\varepsilon_{vC},$ respectively.  Each node $h_i^k$ along the path $\mathcal{H}^k$ can compress the data generated by leaf node $k$ with a \emph{data reduction rate} $\delta_{k,i}$ (ratio of the outgoing data from a node to the incoming data), where $0<\delta_{k, i}\leq 1,$ $\forall i, k.$  The reduction rate characterizes the degree to which a node can compress the received data, which plays an important role for determining the QoI. 

\begin{table}
	\centering
	\caption{Summary of notations}
	\vspace{-0.1in}
	\begin{tabular}{|l|p{9cm}|}
		\hline
		\textbf{Notation} & \textbf{Description} \\ \hline
		$y_{k}$ 	&  number of data (bits) generated at node $k$ \\ \hline
		$y_{v}$ 	&  number of data (bits) present at node $v$ where $y_{v}=\prod_{j=h(k)}^{h(v)}\delta_{k,j}y_{k}$ \\ \hline
		$\delta_{k,v}$	& reduction rate at node $v$, is the ratio of amount of output data to input data  \\ \hline
		$\gamma$	& the QoI threshold    \\ \hline
		$\varepsilon_{vR}$ & per-bit reception cost of node $v$   \\ \hline
		$\varepsilon_{vT}$ & per-bit transmission cost of node $v$   \\ \hline
		$\varepsilon_{vC}$& per-bit compression cost of node $v$ \\ \hline
		$b_{k, v}$	& $1$ if node $v$ caches the data from leaf node $k$; otherwise $0$ \\ \hline
		$S_v$ & storage capacity of node $v$ \\ \hline
		$w_{ca}$ & caching power efficiency  \\  \hline
		$R_k$ & request rate for data from node $k$\\ \hline
		$N$ & total number of nodes in the network \\ \hline
		$C_v$ &set of leaf nodes that are descendants of node $v$  \\  \hline
		$T$	& time length that data are cached\\ \hline
		$\phi^u$ & upper bound of the objective function  \\ \hline
		$\mathcal{L}$	& list of  regions \\ \hline
		$\mathcal{R}$ & any sub-region in $\mathcal{L} $  \\ \hline
		$\phi^{\mathcal{R}, u}$	& upper bound on the objective function in subregion $\mathcal{R}$ \\ \hline
		$\phi^{\mathcal{R}, l}$	& lower bound on the objective function in subregion $\mathcal{R}$  \\ \hline
		$\epsilon$	& difference between the upper and lower bound   \\ \hline
	\end{tabular}
	\label{tab:notations}
	\vspace{-0.2in}
\end{table}



The higher the value of $\delta_{k, i}$, the lower the compression will be, and vice versa. The higher the degree of data compression, the larger will be the amount of energy consumed by compression.  Similarly, caching the data  closer to the sink node may reduce the transmission cost for serving the request, however, each node only has finite storage capacity. We study the tradeoff among the energy consumed at each node for transmitting, compressing and caching the data.  


Denote the total energy consumption at node $v$ as $E_v$, which consists of the reception cost $E_{vR}$,  transmission cost $E_{vT}$, computation cost $E_{vC}$ and storage (caching) cost $E_{vS}$; it takes the form 
\vspace{-0.05in}
\begin{align}
	E_v=E_{vR}+E_{vT}+E_{vC}+E_{vS},
\end{align}
\vspace{-0.05in}
where 
\vspace{-0.05in}
\begin{align}
	&E_{vR}=y_{v}\varepsilon_{vR}, &E_{vT}=y_{v}\varepsilon_{vT}\delta_{v}, \nonumber\displaybreak[0]\\
	&E_{vC}=y_{v}\varepsilon_{vC}l_v(\delta_v),  &E_{vS}=w_{ca}y_{v}T. 
\end{align}

Here, $l_v(\delta_v)$ captures the computation energy. As computation energy increases with the degree of compression, we assume that $l_v(\delta_v)$ is a continuous, decreasing and differentiable function of the reduction rate.  One candidate function is $l_v(\delta_v)=1/\delta_{v}-1$ \cite{nazemi2016qoi,laporta2012}.  Moreover, we consider an energy-proportional model \cite{choi2012network} for caching, i.e., $E_{vS}=w_{ca}y_{v}T$ if the received data $y_v$ is cached for a duration of $T$  where $w_{ca}$ represents the power efficiency of caching,  which strongly depends on the storage hardware technology. W.l.o.g., $w_{ca}$ is assumed to be identical for all the nodes.  {For simplicity, denote 
	\vspace{-0.2in}
	\begin{align}
		f(\delta_v)= \varepsilon_{vR}+\varepsilon_{vT}\delta_{v}+\varepsilon_{vC}l_v(\delta_v),
	\end{align}
	%\vspace{-0.05in}
	as the sum of per-bit reception, transmission and compression cost at node $v$ per unit time.}

During  time period  $T$, we assume that there are $R_{k}$ requests at the sink node $s$ for data $y_k$ generated by leaf node $k$\footnote{As motivated in Section~\ref{sec:intro}, a large number of agents may desire the same information, hence there are multiple requests for the same data.}.  We set the boolean variable $b_{k,i}$ to $1$ if the data from node $k$ is stored along the path $\mathcal{H}^k$  at node $h_i^k,$ otherwise it equals $0$. For ease of notation, we denote $b_{k, h(k)}$ by $b_k,$  $f_{k,h(k)} \triangleq f_k$ and $\delta_{k,h(k)}\triangleq \delta_k.$   %A boolean variable $a_{k,i}$ equals $1$ if the data from node $k$ is transmitted by node $h_i$ on the path $\mathcal{H}^k$, otherwise it equals $0$.
Let $C_v$ denote the set of leaf nodes $k \in \mathcal{K}$ that are descendants of node $v$.

%Furthermore, we assume that the network is structured i.e. the sink node knows which unique path to follow for a specific request. 
We also assume that the {energy cost for searching for data at different nodes} in the network is negligible \cite{nazemi2016qoi, ioannidis16}.
For  ease of exposition,  the parameters used throughout this paper are summarized in Table~\ref{tab:notations}.






==> 04-spatial-new.tex <==
%
%%There are two broad classes of solutions for non-convex MINLP problems namely deterministic and stochastic methods. Since discussing the advantages and disadvantages of both classes is beyond the scope of this paper, interested readers are refered to \cite{floudas2013deterministic} for detailed discussion. To solve our optimization problem, we use a deteministic approach based on spatial branch-and-bound method that is widely used for such  problems. Our proposed approach is a variant of Smith's spatial branch-and-bound method \cite{smith1999symbolic}, which requires reformulating the original problem in \eqref{eq:optimization} into an exact problem \eqref{eq:exactproblem} using \emph{Symbolic reformulation} \cite{smith1996global} which we discuss in the next subsection. 
%
%%\blue{There are two basic methods, deterministic and stochastic, to solve non-convex MINLP problems. The pro and con are discussed in \cite{floudas2013deterministic}. In this paper, we adopt a deterministic method. \red{give more reasons?} }
%
%%In this section, we present a variant of the Spatial Brand-and-Bound algorithm (V-SBB)\red{, that requires \eqref{eq:optimization} to be transformed into an equivalent problem through \emph{Symbolic Reformulation}\cite{smith1996global}. Symbolic Reformulation  allows to reformulate a class of MINLP problems (including \eqref{eq:optimization}) into \eqref{eq:genericre}. The new decision variable vector $\bf w$ consists of the continuous and discrete variables in original problem such as $\delta$ and $b$ in \eqref{eq:optimization} along with added auxiliary variables that arise during the reformulation process. Since \eqref{eq:optimization} consists of bilinear and linear fractional terms, the symbolic reformulation procedure replaces them with new auxiliary variables $w_i$ and incorporates the relationship between the original bilinear, linear fractional terms and the new auxiliary variables as constraint i.e. the third and fourth constraints in \eqref{eq:genericre}. The sets $\tau_{bt}$ and $\tau_{lft}$ consist of all such relationships that arise as a result of reformulation.} 
%
%
%%\subsection{Symbolic Reformulation}
%%We first transform our original MINLP problem \eqref{eq:optimization} into an equivalent problem through symbolic reformulation \cite{smith1996global} as V-SBB requires the optimization problem to be in the form {as in} \eqref{eq:exactproblem}. 
%%\red{Symbolic reformulation through }
%% Under symbolic reformulation, a set of linear constraints and new auxiliary variables are introduced to replace the bi-linear/linear fractional terms in \eqref{eq:optimization}, which eliminate the non-convexities and non-linearities in the objective function and set of constraints in the original problem, and transform them to  {new auxiliary variables and constraints. For example, replacing the \emph{monomial} term $\prod_{i=0}^{h(k)}\delta_{k, i}$ with an auxiliary variable $\overline{w_{k,j}^{C_1}}$ makes the first constraint in \eqref{eq:exactproblem} linear while it is signomial (non-convex) in \eqref{eq:optimization}. }%sets of bilinear $\mathcal{T}_{\text{bt}}$ and linear fractional terms  $\mathcal{T}_{\text{lft}}$.
%  
%%Due to space constraints, we skip the detailed steps of the reformulation, which are available in \cite{faheemjian17}.  {The reformulated problem contains the original linear constraints and variables along with newly added linear constraints (as a result of symbolic reformulation) and variables.} The new variable vector $\mathbf{w}$ consists of continuous and discrete variables in the original MINLP, as well as other auxiliary variables introduced as a result of the reformulation. The objective function $w_f$ {is linear in the auxiliary variables}. %\red{\bf [Comments: Detailed steps can be put in tech report]} Instead, we directly present the reformulated problem as follows
%\red{\bf [Comments: add more explanations of the variables in (6)]}
%
%
In this section, we present a variant of the Spatial Brand-and-Bound algorithm (V-SBB).  Instead of solving the MINLP problem~(\ref{eq:optimization}) directly, we use V-SBB to solve a \emph{standard form} of the original MINLP.   We first introduce the \emph{Symbolic Reformulation}\cite{smith1996global} method that reformulates the MINLP~(\ref{eq:optimization}) into a standard form needed by V-SBB.
\begin{definition}
%\red{The equivalent of any standard MINLP problem can be written as}
A MINLP problem is said to be in a \emph{standard form} if it can be written as 
\begin{align}
\min_{\boldsymbol w}\quad &\boldsymbol w_{\text{obj}}\nonumber \\
\text{s.t.} \quad&\mathbf{Aw=b}, \nonumber\displaybreak[0]\\
&\mathbf{w}^l\leq \mathbf{w}\leq \mathbf{w}^U,  \nonumber\\
& \mathbf{w}_k \equiv \mathbf{w}_i \mathbf{w}_j,\quad \; \forall(i,j,k) \;\in \; \mathcal{T}_{\text{bt}},  \nonumber\displaybreak[1]\\
& \mathbf{w}_k \equiv \mathbf{w}_i/\mathbf{w}_j,\quad  \; \forall(i,j,k) \;\in \; \mathcal{T}_{\text{lft}},
\label{eq:genericre}
\end{align}
where the vector of variables $\boldsymbol w$ consists of continuous and discrete variables in the original MINLP.  The sets $\tau_{\text{bt}}$ and $\tau_{\text{lft}}$ contain all relationships that arise in the reformulation. $\boldsymbol A$ and $\boldsymbol b$ are a matrix and a vector of real coefficients, respectively.  The index $\text{obj}$ denotes the position of a single variable corresponding to the objective function value within the vector $\boldsymbol w.$ 
%as well as slack variables that have been introduced to convert the inequality constraints \red{\bf [comment: We are not using any slack variables as Leo in his phd thesis pointed out that Smith's method can work without any need for slack variables]} in the original MINLP to equalities and any auxiliary continuous variables introduced during the reformulation. The sets $\tau_{\text{bt}}$ and $\tau_{\text{lft}}$ contain all such relationships that arise in the reformulation. $A$ and $b$ are a matrix and a vector of real coefficients, respectively. \red{The index $\text{obj}$ denotes the position of a single variable corresponding to the objective function value within the vector $\boldsymbol w.$}
\end{definition}


%We first show that the MINLP problem~(\ref{eq:optimization}) can be converted to a \emph{standard form}.
\begin{theorem}
The non-convex MINLP problem~(\ref{eq:optimization}) can be  transformed into a standard form.
\end{theorem}
Due to space constraints, we relegate detailed reformulations and standard form of~(\ref{eq:optimization}) to \cite{faheemjian17}. 

Here, we give an example to illustrate the above reformulation process.


\begin{example}
	\normalfont
We consider $k=1$ and $h(k)=1$ in~(\ref{eq:optimization}), i.e., one leaf node and one sink node. Then~(\ref{eq:servingcost}) and~(\ref{eq:cachretrievecost}) reduce to 
\begin{small}
\begin{align}
&E_1^C=y_1f(\delta_{1, 0})\delta_{1,1}+y_1f(\delta_{1,1}), \nonumber\\
&E_1^R=y_1(R_1-1)\left[f(\delta_{1, 0}\delta_{1,1}+\delta_{1,0} \delta_{1,1}b_{1,0}(w_{ca}T+\delta_{1T})\right]\nonumber\\
&+y_1(R_1-1)\left[f(\delta_{1, 1}(1-b_{1,0})+\delta_{1,0} \delta_{1,1}b_{1,1}(w_{ca}T+\delta_{1T})\right],
\end{align}
\end{small}
and non-convex MINLP problem is 
\begin{align}\label{eq:opt-example2nodes}
 \min_{\boldsymbol \delta, \boldsymbol b}\quad &E^{\text{total}}(\boldsymbol{\delta},\boldsymbol{b})=E_1^C+E_1^R\nonumber\\
 \text{s.t.} \quad& y_1\delta_{1,0}\delta_{1,1}\geq\gamma, \nonumber\\
 &b_{1,0}, b_{1,1}\in\{0, 1\}, \nonumber\\
 &b_{1,0}y_1\delta_{1,0}\delta_{1,1}\leq S_0,\nonumber\\
 &b_{1,1}y_1\delta_{1,1}\leq S_1,\nonumber\\
 &b_{1,0}+b_{1,1}\leq 1.
\end{align}
%Given the original non-convex MINLP in~(\ref{eq:optimization}) with $k=1$ and $h(k)=1$. 
$\delta_{1, 0} \delta_{1, 1}$ is a bilinear term.  Based on symbolic reformulation rules (see \cite{faheemjian17} for details), a new bilinear auxiliary variable $w_{1,0}^{\text{bt}}$ needs to be added. % where the superscript $\text{bt}$ denotes bilinear terms.  
 The first constraint in \eqref{eq:opt-example2nodes} is then transformed into $ y_{1} w_{1,0}^{\text{bt}} \geq \gamma,$ which is linear in auxiliary variable $w_{1,0}^{\text{bt}}$. %and $w_{1,0}^b = \delta_{1, 1}\times \delta_{1,0}$ as a constraint. 
Similarly, we add $w_{1,0}^{\text{lft}}$ for linear-fractional term $\delta_{1, 1}/\delta_{1, 0}$ that appears in $f(\cdot).$ % where the superscript $\text{f}$ denotes fractional terms. %and add $w_{1,0}^f=\frac{\delta_{1, 1}}{\delta_{1, 0}}$ as a constraint. 
$b_{1,0}\delta_{1, 0}\delta_{1, 1}$ in the third constraint of \eqref{eq:opt-example2nodes} is a tri-linear term.  Since $\delta_{1, 0}\delta_{1, 1}$ is replaced by $w_{1,0}^{\text{bt}}$, we obtain a bilinear term $b_{1,0}w_{1,0}^{\text{bt}}$.  Again,  based on symbolic reformulation rules, $b_{1,0}w_{1,0}^{\text{bt}}$ is replaced by a new auxiliary variable $\overline{w}_{1,0}^{\text{bt}}$. % and we also add a constraint $\overline{w}_{1,0}^b=b_{1,0}w_{1,0}^b$. 
Similarly we add new auxiliary variables $\tilde{w}_{1,1}^{\text{b}}, \tilde{w}_{1,0}^{\text{bt}},$ and $\tilde{w}_{1,0}^{\text{lft}}$.  The objective function in~(\ref{eq:opt-example2nodes}) can be then expressed as a function of these new auxiliary variables.  Therefore, the standard form of \eqref{eq:opt-example2nodes} is 
%Using this approach, we transform \eqref{eq:opt-example2nodes} into \eqref{eq:example2nodes}. 
	%New auxiliary variables like $\overline{w}_{k,j}^{C_1}, \overline{w}_{k,i}^{C_2}, \overline{w}_{k,a}, w^b_{k,i}, w^f_{k,i}, \overline{w}_{k,i}^{C''_2}   ,\overline{w}_{k,a}, \overline{w}_{k,\beta}^{C'_2}, \overline{w}_{k,i}^{C_2}$  are introduced to replace the non-convex and non-linear terms in \eqref{eq:optimization} using the same idea as in our aforementioned example. 
 %\red{\bf[Comments: can you rewrite this paragraph to give a detailed explanations of all the variables used below]}
%Then the standard form of~(\ref{eq:opt-example2nodes}) is 
\begin{small}
\begin{align}
 \min_{\boldsymbol \delta, \boldsymbol b}\quad & w_{\text{obj}}
 \nonumber \\
\text{s.t.} \quad& y_{1} w_{1,0}^{\text{bt}} \geq \gamma, \nonumber\\
%&  b_{k,i}\in\{0,1\}, \forall  k\in\mathcal{K}, i=0, \cdots, h(k),  \nonumber\displaybreak[1]\\
&  b_{1,0}, b_{1, 1}\in\{0,1\},  \nonumber\displaybreak[0] \\
& y_{1} \overline{w}_{1,0}^{\text{bt}}\leq S_0, \nonumber\\
& y_{1} \tilde{w}_{1,1}^{\text{bt}}\leq S_1, \nonumber\\
%& \sum_{i=0}^{h(k)}b_{k,i} \leq 1,\forall k\in\mathcal{K}, \displaybreak[3] \nonumber \\
 &b_{1,0}+b_{1, 1}\leq 1, \nonumber\\
& w_{1,0}^{\text{bt}} = \delta_{1, 1}\times \delta_{1,0}, \nonumber\\
& w_{1,0}^{\text{lft}} = \delta_{1, 1}/\delta_{1,0}, \nonumber\\
& \overline{w}_{1,0}^{\text{bt}} = b_{1,0} \times w_{1,0}^b, \nonumber\\
& \tilde{w}_{1,1}^{\text{bt}} = b_{1, 1} \times \delta_{1, 1}, \nonumber\displaybreak[1] \\
&  \tilde{w}_{1,0}^{\text{bt}}= \delta_{1, 1}\times b_{1,0},\nonumber \displaybreak[2] \\
&  \tilde{w}_{1,0}^{\text{lft}}=  b_{1,0}/\delta_{1, 1},\nonumber\displaybreak[3] \\
& w_{\text{obj}} = y_1 \varepsilon_{1R} \delta_{1,1}+\varepsilon_{1T}y_1 w_{1,0}^{\text{bt}}+y_1 \varepsilon_{1C} w_{1,0}^{\text{lft}}-y_1 \varepsilon_{1C} \delta_{1, 1}\nonumber\displaybreak[4] \\
&+y_1 \varepsilon_{1R} +\varepsilon_{1T} y_1 \delta_{1, 1} +y_1 \varepsilon_{1C}/\delta_{1,1}-y_1 \varepsilon_{1C}+ y_1R_1\varepsilon_{1R}\delta_{1,0} \nonumber \\
&+y_1R_1\varepsilon_{1T}w_{1,0}^{\text{bt}}+y_1R_1\varepsilon_{1C}w_{1,0}^{\text{lft}} -y_1R_1\varepsilon_{1C}\delta_{1,1}-y_1R_1\delta_{1,1}\nonumber\\
&-y_1\varepsilon_{1T}w_{1,0}^{\text{bt}}- y_1\varepsilon_{1C}w_{1,0}^{\text{lft}}+y_1\varepsilon_{1C}\delta_{1, 1}+y_1R_1w_{ca}T\overline{w}_{1,0}^{\text{bt}}\nonumber \\ 
&  +y_1R_1\varepsilon_{1T}\overline{w}_{1,0}^{\text{bt}}-y_1w_{ca}T\overline{w}_{1,0}^{\text{bt}}-y_1\varepsilon_{1T}\overline{w}_{1,0}^{\text{bt}}+ y_1 R_1 \varepsilon_{1R} \nonumber \\
& +y_1R_1\varepsilon_{1T}\delta_{1,1} + y_1R_1\varepsilon_{1C}/\delta_{1, 1}-y_1R_1\varepsilon_{1C}-y_1\varepsilon_{1C}\nonumber\\
&-y_1\varepsilon_{1T}\delta_{1}-y_1\varepsilon_{1C}/\delta_{1,1}+y_1\varepsilon_{1C}-y_1R_1\varepsilon_{1R}b_{1,0} \nonumber \\
& -y_1R_1\varepsilon_{1T}\tilde{w}_{1,0}^{\text{bt}}-y_1R_1\varepsilon_{1C}\tilde{w}_{1,0}^{\text{lft}}+y_1R_1\varepsilon_{1C}b_{1,0}+y_1\varepsilon_{1R}b_{1,0}\nonumber\\
&+y_1\varepsilon_{1T}\tilde{w}_{1,0}^{\text{bt}}+y_1\varepsilon_{1C}\tilde{w}_{1,0}^{\text{lft}}-y_1\varepsilon_{1C}b_{1,0}+y_1R_1w_{ca}T\tilde{w}_{1,1}^{\text{bt}}\nonumber\\
&+y_1R_1\varepsilon_{1T}\tilde{w}_{1,1}^{\text{bt}}-y_1w_{ca}T\tilde{w}_{1,1}^{\text{bt}}-y_1\varepsilon_{1T}b_{1,1}.
\label{eq:example2nodes}
\end{align}
\end{small}
\end{example}
Through this reformulation, the non-convex and non-linear terms in the original problem are transformed into bilinear and linear fractional terms, which can be easily used to compute the lower bound of each region in V-SBB, which are discussed in details later.  This is the reason V-SBB requires reformulating the original problem into a standard form.
%\red{%The advantage of reformulation is that it removes non-convexities and non-linearities from the original formulation and contain them in the sets $\tau_{\text{bt}}$ and $\tau_{\text{lft}}$.
	  %V-SBB involves calculating the lower bound for each region (discussed in detail later) by solving a convex relaxation of the problem; however, obtaining a convex relaxation for \eqref{eq:optimization} is tedious due to the presence of non-linear terms. Since the reformulated problem \eqref{eq:example2nodes} consists of bilinear and linear fractional terms, McCormick's linear over and under-estimators (see \cite{faheemjian17} for details) can be easily used to obtain the convex relaxations. This is why V-SBB requires reformulating the original problem.    }



%\red{ We provide a brief discussion on symbolic reformulation of \eqref{eq:optimization} here, however interested readers are referred to \cite{faheemjian17} for detailed description of reformulating \cite{faheemjian17}. As an example, we take the term $\prod_{i=0}^{h(k)}\delta_{k, i}$, and symbolically reformulate it into an auxiliary variable $\overline{w}_{k,j}^{C_1}$ where $j=h(k)-1$. For sake of simplicity, we assume that $h(k)$ is 1. Then $\prod_{i=0}^{h(k)}\delta_{k, i}=\delta_{k, 0} \times \delta_{k, 1}$ is a bilinear term. Based on the rules of symbolic reformulation (see \cite{faheemjian17} for details), this requires adding a new bilinear auxiliary variable $\overline{w}_{k,0}^{C_1}$. The second constraint in \eqref{eq:optimization} is transformed into $ \sum_{k \in C_v}y_k {\overline{w}_{k,i}^{C_2}}\leq S_v, \forall \; v \in V,$ which is linear in the auxiliary variable. Furthermore we introduce another constraint $\overline{w}_{k,0}^{C_1}=\prod_{i=0}^{1}\delta_{k, i}$. Using this approach, we transform \eqref{eq:optimization} into \eqref{eq:exactproblem}. New auxiliary variables like $\overline{w}_{k,j}^{C_1}, \overline{w}_{k,i}^{C_2}, \overline{w}_{k,a}, w^b_{k,i}, w^f_{k,i}, \overline{w}_{k,i}^{C''_2}   ,\overline{w}_{k,a}, \overline{w}_{k,\beta}^{C'_2}, \overline{w}_{k,i}^{C_2}$  are introduced to replace the non-convex and non-linear terms in \eqref{eq:optimization} using the same idea as in our aforementioned example. }


%\begin{small}
%	\begin{align}
%	\min_{w}\quad &w_{f}\nonumber \\
%	\text{s.t.} \quad&\sum_{k\in \mathcal{K}}y_{k} {\overline{w}_{k,j}^{C_1}}\geq\gamma, \nonumber\\
%	&  \sum_{k \in C_v}y_k {\overline{w}_{k,i}^{C_2}}\leq S_v, \forall \; v \in V, \nonumber \\
%	& \sum_{i=0}^{h(k)}b_{k,i} \leq 1,\forall k\in\mathcal{K},  \nonumber \\
%	&  b_{k,i}\in\{0,1\}, \forall  k\in\mathcal{K}, i=0, \cdots, h(k),  \nonumber\\
%	&	\mathbf{w}^l\leq \mathbf{w}\leq \mathbf{w}^U,\; \forall  k\in\mathcal{K}, i=0, \cdots, h(k),  \nonumber \\
%	& w_{k,i}^b=\delta_{k, i}\times \overline{w}_{k,a}, \;  \forall  k\in\mathcal{K}, i=0, \cdots, h(k),  \nonumber \\
%	& w_{k,i}^f=\frac{\overline{w}_{k,a}}{\delta_{k, i}} , \;  \forall  k\in\mathcal{K}, i=0, \cdots, h(k), \nonumber \\
%	& y_k b_{k,i}-\overline{w}_{k,i}^{C''_2}=0 , \;  \forall  k\in\mathcal{K}, i=0, \cdots, h(k), \nonumber \\
%	& \overline{w}_{k,i}^{C_2}= \overline{w}_{k,i}^{C''_2} \times \overline{w}_{k,\beta}^{C'_2} , \;  \forall  k\in\mathcal{K}, i=0, \cdots, h(k), \nonumber \\
%	& \sum_{j=0}^{i-1}b_{k,j} - \widetilde{w}_{k,i}=0 , \;  \forall  k\in\mathcal{K}, i=0, \cdots, h(k), \nonumber\\
%	& \overline{\overline{w}}_{k,i}=\overline{w}_{k,a} \times \widetilde{w}_{k,i} , \;  \forall  k\in\mathcal{K}, i=0, \cdots, h(k),  \nonumber\\
%	& \overline{w}_{k,i}^b=w_{k,i}^b \times \widetilde{w}_{k,i} , \;  \forall  k\in\mathcal{K}, i=0, \cdots, h(k),  \nonumber \\
%	& \overline{w}_{k,i}^f=w_{k,i}^f \times \widetilde{w}_{k,i}, \;  \forall  k\in\mathcal{K}, i=0, \cdots, h(k),  \nonumber\\
%	& \prod_{m=i+1}^{h(k)}\delta_{k, m}=\overline{w}_{k,\underbrace{h(k)-2-i}_a}\nonumber\\
%	&\qquad\qquad\quad=\begin{cases}
%	\delta_{k,h(k)} \times \delta_{k,h(k)-1},& \forall a=0 \\ 
%	\overline{w}_{k,a-1}\times \delta_{k,m}, &  m+a=h(k)-1 \\ 
%	\delta_{k,h(k)}, & \forall i=h(k)-1, 
%	\end{cases} \nonumber \\
%	& \prod_{i=0}^{h(k)}\delta_{k, i}=\overline{w}_{k,\underbrace{h(k)-1}_j}^{C_1}\nonumber\\
%	&\qquad\qquad= 
%	\begin{cases}
%	\delta_{k,h(k)} \times \delta_{k,h(k)-1},& \forall j=0 \\ 
%	\overline{w}_{k,j-1}^{C_1}\times \delta_{k,j+1}, &  \forall j=1 \cdots h(k)-1 \\ 
%	\delta_{k,h(k)}, & \forall i=h(k),
%	\end{cases} \nonumber\displaybreak[0]   \\
%	& \prod_{j=h(k)}^{h(v)}\delta_{k,j}={\overline{w}_{k,\underbrace{\tau-2}_\beta}^{C'_2}=}
%	\begin{cases}
%	\delta_{k,h(k)} \times \delta_{k,h(k)-1},& \forall \beta=0 \\ 
%	\overline{w}_{k,j-1}^{C_1}\times \delta_{k,j+1}, &  \forall \beta > 0 \\ 
%	\delta_{k,h(k)}, & \forall \beta <0,
%	\end{cases} \nonumber \displaybreak[1] \\ 
%	&w_f=\sum_{k \in \mathcal{K}}\sum_{i=0}^{h(k)}y_k \Bigg(\bigg( \varepsilon_{kR}\overline{w}_{k,a}+\varepsilon_{kT}w_{k,i}^b+\varepsilon_{kC} w_{k,i}^f  \nonumber\displaybreak[2]\\
%	&\qquad\qquad\qquad- \varepsilon_{kc}\overline{w}_{ka}\bigg)+A+B\Bigg),\nonumber \displaybreak[3]\\ 
%	& A=\varepsilon_{kR}R_k\overline{w}_{k,a}+\varepsilon_{kT}w_{k,i}^b+\varepsilon_{kc}R_kw_{k,i}^f-\varepsilon_{kC}R_k\overline{w}_{k,a} \nonumber\\
%	&\qquad\qquad- \varepsilon_{kR}\overline{w}_{k,a}-\varepsilon_{kT}w_{k,i}^b-\varepsilon_{kC}w_{k,i}^f+\varepsilon_{kC}\overline{w}_{k,a}, \nonumber \displaybreak[4]\\
%	& B=-\varepsilon_{kR}R_k \overline{\overline{w}}_{k,i}-\varepsilon_{kT}R_k \overline{w}_{k,i}^b-\varepsilon_{kc}R_k\overline{w}_{k,i}^f\nonumber\\
%	&+  \varepsilon_{kC}R_k\overline{\overline{w}}_{k,i}+\varepsilon_{kR}\overline{\overline{w}}_{k,i}+\varepsilon_{kT}\overline{w}_{k,i}^b+\varepsilon_{kC}\overline{w}_{k,i}^f- \varepsilon_{kC}\overline{\overline{w}}_{k,i}.
%	\label{eq:exactproblem}
%	\end{align}
%\end{small}


%\begin{strip}



%\red{The sets $\mathcal{T}_{bt}$ and $\mathcal{T}_{lft}$  contain the bilinear, linear fractional and auxiliary terms that 
%where $\mathcal{T}_{bt}$ and $\mathcal{T}_{lft}$ are the resultant sets of bilinear and linear fractional terms, respectively.  
	  %This reformulation ensures that the new objective function and the first constraint in~(\ref{eq:exactproblem}) are linear, and all non-convexities and non-linearities in the original MINLP are absorbed by the sets $\mathcal{T}_{\text{bt}}$ and $\mathcal{T}_{\text{lft}}$.  For example, if the original problem variables \emph{x,y} are present as product $xy$ in the original problem, they will be replaced by a  auxiliary variable $w_i\equiv xy$ in the reformulated problem, \red{which is now linear in $w_i$} where $w_i\equiv xy \in \mathcal{T}_{\text{bt}}$. %and  $\mathcal{T}_{bt}$ will reflect this relationship between $w,x \; and \; y.$ 

\begin{theorem}
%Reformulated problem~(\ref{eq:exactproblem}) and the original MINLP \eqref{eq:optimization} are equivalent.}
Reformulated problem and the original MINLP are equivalent.
\end{theorem}
Proof is available in \cite{faheemjian17}.

Due to the reformulation, the number of variables in the reformulated problem is larger than in the original MINLP. In the following, we show that the number of auxiliary variables that arise from symbolic reformulation is bounded. 
\begin{rem}
	\label{thm:numberofvariables}
The number of auxiliary variables in the symbolic reformulation is $O(n^2),$ where $n=2M$ is the number of variables in the original  formulation.
\end{rem}
%\begin{proof}
From \cite{smith1999symbolic}, a way to transform a general form optimization problem %\eqref{eq:generaloptimizationform} 
into a standard form \eqref{eq:genericre} is through basic arithmetic operations on original variables. To be more specific, any algebraic expression results from the basic operators including the five basic binary operators, i.e., addition, subtraction, multiplication, division and exponentiation, and the unary operators, i.e., logarithms etc.  Therefore, in order to construct a standard problem consisting of simple terms corresponding to these binary or unary operations, new variables need to be added corresponding to these operations.  From the symbolic reformulation process \cite{smith1999symbolic, smith1996optimal, liberti2004reformulation}, any added variable results from the basic operations between two (including possibly the same) original variables or added variables. Hence, based on the basic operations, there are at most $n^2$ combinations of these variables, given that there are $n$ variables in the original problem \eqref{eq:optimization}. Therefore, the number of added variables in the symbolic reformulation is bounded as $O(n^2).$
%\end{proof}
In the remainder of this section, we present the V-SBB to solve the equivalent problem. % defined in~(\ref{eq:exactproblem}).% which is equivalent to the original MINLP problem in \eqref{eq:optimization}. 


\subsection{Variant of Spatial Branch-and-Bound Algorithm}
In contrast with conventional SBB, our newly proposed V-SBB eliminates the bound-tightening steps. This has two advantages: (i) bound tightening step does not always guarantee faster convergence; (ii) removal significantly reduces the computational complexity of the algorithm. 
%Our proposed V-SBB algorithm is a computationally efficient variant of the conventional SBB \cite{smith1999symbolic} from two perspectives: (i) We eliminate the bounds tightening steps, which not only slow down the branch and bound process, but also does not guarantee any faster convergence \cite{liberti2004phdthesis}; (ii) the computational complexity of our V-SBB is much reduced compared to the original SBB \cite{smith1999symbolic}. 
 Algorithm \ref{algo:sbnb} gives an overview of V-SBB.  
 %\blue{Our proposed V-SBB is \red{computationally efficient version of the} algorithm proposed in \cite{smith1999symbolic}. \red{We improve the computational efficiency by eliminating the bounds tightening step in the traditional SBB because i) bounds tightening always does not result in faster convergence \cite{liberti2004phdthesis} (which is the case for our formulation); ii) tightening the bounds will neccesitate  calculating the lower bound of a subregion $\mathcal{R} \in \mathcal{L}$ twice in the same iteration.}} 
	%	(i) First, we do not use any bounds tightening steps, which not only slow down the branch and bound process, but also not guarantee any faster convergence \cite{liberti2004phdthesis}; (ii) Second, since there is no need to tighten the bounds again, the computational complexity of our V-SBB is much reduced compared to the original SBB \cite{smith1999symbolic}. } \red{\bf [only these two differences?] \emph{\blue{\bf{yes these are the two major differences between the two techniques as spatial branch and bound has the same steps. }}}}
%The proposed spatial branch-and-bound method is a variant of the method proposed in \cite{smith1999symbolic} and is primarily tuned for solving our optimization problem \eqref{eq:exactproblem} that is also the solution of \eqref{eq:optimization}. \red{ Our algorithm is  different from \cite{smith1999symbolic} because} 
%	\begin{itemize}
%		\item \red{We do not use any bounds tighening steps as it does not always guarantee faster convergence \cite{liberti2004phdthesis} and in case of our problem slowed down the process. 
%		\item   By eliminating the bounds tightening step, we do not need to calculate the lower bound again separately and utilize the lower bound obtained in Step 2 for the chosen region $\mathcal{R}$, hence reducing the computational complexity of the algorithm}.
%	\end{itemize}
%	It is worth mentioning here that unlike \cite{smith1999symbolic}, 
 %Algorithm \ref{algo:sbnb} gives an overview of our V-SBB.  Here, we briefly describe the key steps due to space limitation. \blue{A thorough explanation of each step is given in [tech report].}
% Algorithm \ref{algo:sbnb} provides an overview of the steps involved in spatial branch-and-bound algorithm. We describe some of the steps in Algorithm \ref{algo:sbnb} in detail below. 
%\subsubsection{Step 2} 
We briefly describe the key steps due to space limitations. A detailed explanation of each step is given in \cite{faheemjian17}.\\
\noindent{\textit{Step $2$:}} 
We use the \emph{least lower bound rule}\footnote{{Select a subregion $\mathcal{R} \in \mathcal{L}$  , whose convex relaxation provides the lowest objective function value}.} to choose a subregion $\mathcal{R}$ from $\mathcal{L}$ %that has the least lower bound 
among all feasible subregions. This lower bound is obtained by solving a convex relaxation of the reformulated problem such as~\eqref{eq:example2nodes}.  McCormick linear over-estimators and underestimators \cite{mccormick1976computability} are used to obtain the convex relaxation for bilinear terms (bt) and linear fractional terms (lft). 
%Since our framework in \eqref{eq:optimization} and \eqref{eq:exactproblem} contains both linear and bilinear fractional terms, we use McCormick linear over-estimators and underestimators \cite{mccormick1976computability} (see Appendix \ref{sec:appendixA}) to obtain a convex relaxation of all such terms.  The resultant problem is a
 This leads to a Mixed Integer Linear Program (MILP), that can be solved by the  \emph{SCIP} solver \cite{achterberg2009scip}.  Denote the optimal solution of this subregion as $\phi^{\mathcal{R},l}$. %to obtain the  explore the optimal solution in this subregion, denoted as $\phi^{\mathcal{R},l}$. 
Note that if the convex relaxation is infeasible or the obtained lower bound is greater than the current upper bound $\phi^u$, we move to \emph{Step $5$}, otherwise we move to \emph{Step $3$}.
%There are a number of approaches that can be used to choose a subregion $\mathcal{R}$ from $\mathcal{L}$ \cite{floudas2013deterministic} however, we use the \emph{least lower bound rule} i.e. we choose a subregion \red{$\mathcal{R} \in \mathcal{L}$} that has the lowest lower bound \red{among all the available subregions}. The lower bound can be obtained by solving a convex relaxation of the problem in \eqref{eq:exactproblem}.  As our optimization problem in \eqref{eq:optimization} and \eqref{eq:exactproblem} contains only bilinear and linear fractional terms, we use McCormick  linear over-estimators and underestimators \cite{mccormick1976computability} (see Appendix \ref{sec:appendixA}) to obtain a convex relaxation of all such terms. The resulting problem is then a Mixed Integer Linear Programming (MILP) problem that we solve using the \emph{SCIP} solver \cite{achterberg2009scip}. The subregion with lowest lower bound is then used as the region to explore for an optimum. The chosen regions' lower bound is used as $\phi^{\mathcal{R},l}$. \red{If the convex relaxation is infeasible or if the obtained lower bound is higher than the existing upper bound $\phi^u$ of the problem, we \emph{fathom} or delete the current region by moving to step 5}.

%\subsubsection{Step 3}
\noindent{\textit{Step $3$:}} 
We compute the upper bound $\phi^{\mathcal{R},u}$ for the subregion $\mathcal{R}$ through local MINLP solver such as \emph{Bonmin} \cite{bonami2008algorithmic}.  If this upper bound cannot be obtained or is greater than $\phi^{u}$,  we move to \emph{Step $4$}. Otherwise, we set it as the current best solution $\phi^{u}$, and delete all other subregions that have higher lower bounds than this region's upper bound.  If the difference between the upper and lower bounds for this subregion is within $\epsilon$-tolerance,  we delete this subregion by moving to \emph{Step $5$}, otherwise move to \emph{Step $4$}.
%In step 3, we calculate the upperbound  $\phi^{\mathcal{R},u}$  for the subregion $\mathcal{R}$ \red{chosen in Step 2}. This can be done in a number of ways (see \cite{smith1999symbolic}), however we use local MINLP solver such as \emph{Bonmin} \cite{bonami2008algorithmic} to obtain a local minimum for the subregion. If the upper bound for the region $\phi^{\mathcal{R},u}$  cannot be obtained or if is is greater than $\phi^{u}$ then we move to Step 4 to further divide the region and search further for a better solution. Otherwise we set it as the current best solution $\phi^{u}$ and delete all the subregions whose lower bound is greater than the obtained upper bound since \red{all such} regions cannot contain the $\varepsilon$-global optimal solution. If the difference between the upper and lowerbound for the region is within the $\varepsilon$-tolerance, the current subregion does not need to be searched further so we fathom \red{the current subregion} by going to step 5, otherwise we move to step 4 for further searching in the space. 



%\subsubsection{Step 4}
\noindent{\textit{Step $4$:}} 
known as the \emph{branching} step, is used to select a variable and its corresponding value at which the region is further divided. % \red{and value for that variable to divide the current region of interest. }% to branching and the value of it under which the region is further divided. 
	Here, we use the variable and value selection rule specified in \cite{smith1996optimal}, under which the variable that causes the maximal reduction in the feasibility gap between the solution of \emph{Step $2$} and the exact problem, is branched on. Then we  partition $\mathcal{R}$ into $\mathcal{R}_{\text{right}}$ and $\mathcal{R}_{\text{left}}$, and add them into $\mathcal{L}$ as well as delete $\mathcal{R}$. 
%Step 4 \red{also known as the branching/partitioning step } helps in partitioning/dividing a region to further refine the \red{search for} solution. In branching step, we select a variable for branching/partitioning as well as the value of the variable at which the region is to be divided. There are a number of different rules and techniques that can be used for branching (see \cite{floudas2013deterministic} for detailed discussion). However, we use the variable selection and value selection rule specified in \cite{smith1996optimal}. 
\begin{comment}
\blue{In order to obtain this, we compute the approximation error for bilinear and linear fractional terms in \eqref{eq:exactproblem} as follows
\begin{align}\label{eq:aperrorbt-lft}
&E^{ijk}_{bt}=|w_k^{S_2}-w_i^{S_2}w_j^{S_2}|, \quad \forall(i,j,k)\in\mathcal{T}_{bt}\nonumber\\
&E^{ijk}_{lft}=\bigg|w_k^{S_2}-\frac{w_i^{S_2}}{w_j^{S_2}}\bigg|,\quad\forall(i,j,k)\in\mathcal{T}_{lft}, 
\end{align}
where $S_2$ is the value of variable obtained in \emph{Step $2$}. \red{\bf [Comments: what is bt, lft? no explanations. Also these should be typed like $\text{bt, lft}$, and $\mathcal{S}$ is usually taken as a set or distribution, so I change the value to $S$.]} The variable with the maximal approximation error is chosen to be branched.  This usually result in two candidate variables for branching i.e. $w_i$ and $w_j$. If one is discrete and the other is continuous, then we branch the discrete variable since only finite number of branches need to be done. Otherwise, we choose the variable $w_b$ given as
\begin{align}\scriptsize
\arg\min\Bigg\{\bigg|0.5-\bigg(\frac{w_i^\mathcal{r}-w_i^{\mathcal{R},l}}{w_i^{\mathcal{R},u}-w_i^{\mathcal{R},l}}\bigg)\bigg|,
	\bigg|0.5-\bigg(\frac{w_j^\mathcal{r}-w_j^{\mathcal{R},l}}{w_j^{\mathcal{R},u}-w_j^{\mathcal{R},l}}\bigg)\bigg| \Bigg\},
\label{eq:variableselection}
\end{align}
whose value $w_b^\mathcal{R}$ is closer to its range's midpoint. Due to space limitation, we give the exact way to compute the midpoint in Appendix.  Thus we can partition $\mathcal{R}$ into $\mathcal{R}_{\text{right}}$ and $\mathcal{R}_{\text{left}}$, and then add them into $\mathcal{L}$ as well as deleting $\mathcal{R}$. }

%We branch on the variable that causes the maximum reduction in the feasibility gap between the \red{solution of} convex relaxation (solution of Step 2) and the exact problem.To do so, the approximation error for the bilinear and linear fractional terms in \eqref{eq:exactproblem} is calculated using \eqref{eq:aperrorbt} and \eqref{eq:aperrorlft} respectively where $\mathcal{S}_2$ means the value of the variable obtained in Step 2. The variable with the maximum approximation error of all is chosen as the branching variable as that tightens the gap between  the relaxation and the exact problem \cite{smith1996optimal}. This results in two candidate variables for branching i.e. $w_i$ and $w_j$. If one of the variables is discrete (binary in our case) and the other is continuous then choose the discrete variable since it will result only in finite number of branches. However, if both variables are of the same type (either binary or continuous), then the branching variable is chosen using \eqref{eq:variableselection} i.e. we choose the variable $w_b$ that has its value $w_b^\mathcal{R}$ closer to its range's midpoint. 
%	\begin{equation}
%	\centering
%	E^{ijk}_{bt}=|w_k^{\mathcal{S}_2}-w_i^{\mathcal{S}_2}w_j^{\mathcal{S}_2}|\; \forall(i,j,k) \;\in \; \mathcal{T}_{bt}
%	\label{eq:aperrorbt}
%	\end{equation}
%	\begin{equation}
%	\centering
%	E^{ijk}_{lft}=\bigg|w_k^{\mathcal{S}_2}-\frac{w_i^{\mathcal{S}_2}}{w_j^{\mathcal{S}_2}}\bigg|\; \forall(i,j,k) \;\in \; \mathcal{T}_{lft}
%	\label{eq:aperrorlft}
%	\end{equation}
%		\begin{align}
%	w_{b}=arg \; min\;\Bigg\{\bigg|0.5-\bigg(\frac{w_i^\mathcal{r}-w_i^{\mathcal{R},l}}{w_i^{\mathcal{R},u}-w_i^{\mathcal{R},l}}\bigg)\bigg|, \nonumber \\
%	\bigg|0.5-\bigg(\frac{w_j^\mathcal{r}-w_j^{\mathcal{R},l}}{w_j^{\mathcal{R},u}-w_j^{\mathcal{R},l}}\bigg)\bigg| \Bigg\}
%	\label{eq:variableselection}
%	\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%Put this in the Appendix%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\red{However,  we first need to obtain the branching value for the candidate variables $w_{bc}^\mathcal{r}$(the value at which to branch).  $w_{bc}^\mathcal{r}$ should be between the upper and lowerbound of the variable in the region i.e. $w_{bc}^{\mathcal{r},l} < w_{bc}^\mathcal{r} < w_{bc}^{\mathcal{r},u}$. The rules for the choice of the branch point have been set in \cite{smith1996optimal}, however we restate them here for sake of completeness. 
%\begin{itemize}
%	\item Set $w_{bc}^\mathcal{r}$ to the value obtained in Step 2 i.e. $w_{bc}^\mathcal{r}:=w_{bc}^{\mathcal{S}_2}$
%	\item If any feasible upper bound $\phi^u=\phi(w_{bc}^*)$ has been obtained and  $w_{bc}^{\mathcal{r},l} < w_{bc}^* < w_{bc}^{\mathcal{r},u}$, then  $w_{bc}^\mathcal{r}:=w_{bc}^*$ and stop the search for the value.
%	\item If step 4 provided an upperbound $\phi^{\mathcal{R},u}$ for the subregion $\mathcal{R}$, then  $w_{bc}^\mathcal{r}:=w_{bc}^\mathcal{R}$
%\end{itemize}
%After obtaining the branch point value, we have all the parameters required for \eqref{eq:variableselection} and can then choose the variable for branching.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\par We  partition the subregion $\mathcal{R}$ into $\mathcal{R}_{right}$ and $\mathcal{R}_{left}$ and add $\mathcal{R}_{right}$, $\mathcal{R}_{left}$ into our region list $\mathcal{L}$. Then we move to \emph{Step 5} and delete the subregion $\mathcal{R}$ from the list $\mathcal{L}$.  


\end{comment}



\subsection{Convergence of V-SBB}
\begin{definition}
%\blue{An algorithm is said to achieving  $\epsilon$-global optimality if the difference between the upper and lower bounds of its solutions are within $\epsilon,$
A solution to an optimization problem is said to be $\epsilon$-global optimal if the difference between this solution and the optimal one is within $\epsilon.$
\end{definition}

\begin{theorem}
Our V-SBB described in Algorithm~\ref{algo:sbnb} converges to an $\epsilon$-global optimal solution of its standard problem given in \cite{faheemjian17}.
\end{theorem}
Though we made critical modifications to obtain our V-SBB algorithm, the proof of convergence follows an argument similar to that of \emph{Branch-and-select} given in \cite{liberti2004phdthesis}.  We present the poof in \cite{faheemjian17} for completeness. 
%The spatial branch-and-bound method guarantees convergence \red{to $\varepsilon-$global optimality}, which has been proven in \cite{liberti2004phdthesis}. However, for sake of completeness, we restate the proof in the Appendix \ref{sec:appendixB}.



\begin{algorithm}
	\begin{algorithmic}[]
		%\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon    instead
		%	\begin{comment}
		%    \textbf{Input:}\\
		%    \textbf{Output:}\\
		%    \textbf{Step 1}: Initialize $\phi^u:=\infty$ and $\mathcal{L}$ to a single domain  \\
		%    \textbf{Step 2}: Choose a subregion $\mathcal{R} \in \mathcal{L}$ \\
		%    \textbf{Step 3}: Obtain the lower bound $\phi^{\mathcal{R},l}$ \\
		%                if
		%	\end{comment}
		%	\State \textbf{Input:} 
		%	\State \textbf{Output:} $\phi^u$
		\State \textbf{Step 1}: Initialize $\phi^u:=\infty$ and $\mathcal{L}$ to a single domain  
		\State \textbf{Step 2}: Choose a subregion $\mathcal{R} \in \mathcal{L}$ using \emph{least lower bound rule}
		\If{ $\mathcal{L}$ = $\emptyset$} Go to Step 6
		%	\State Go to Step 6
		\EndIf
		\If{ for chosen region $\mathcal{R}$,  $\phi^{\mathcal{R},l}$ is infeasible or $\phi^{\mathcal{R},l}\geq \phi^u-\varepsilon$} Go to Step 5
		%	\State Go to Step 5
		\EndIf
		%	\Else { Go to Step 3}
		%	\State		Go to step 3
		
		%	\State  \textbf{Step 3}: Obtain the lower bound $\phi^{\mathcal{R},l}$ 
		
		%	\Else {Go to Step 4:}
		%	\EndIf 
		\State \textbf{Step 3}: Obtain the upper bound $\phi^{\mathcal{R},u}$ 
		\If{upper bound cannot be obtained or if $\phi^{\mathcal{R},u}>\phi^u$} Go to Step 4
		%	\State Go to Step 4
		\Else{ $\phi^u:=$$\phi^{\mathcal{R},u}$} and, from the list $\mathcal{L}$, delete all subregions $\mathcal{S} \in \mathcal{L}$ such that $\phi^{\mathcal{S},l}\geq \phi^u-\epsilon$
		\EndIf
		\If{$\phi^{\mathcal{R},u}-\phi^{\mathcal{R},l}\leq \epsilon$} Go to Step 5
		%\State   Go to Step 5
		\EndIf
		\State \textbf{Step 4}: Partition  $\mathcal{R}$ into new subregions  $\mathcal{R}_{\text{right}}$ and  $\mathcal{R}_{\text{left}}$
		\State \textbf{Step 5}: Delete $\mathcal{R}$ from $\mathcal{L}$ and go to Step 2
		\State \textbf{Step 6}: Terminate Search
		\If{$\phi^u=\infty$}  Problem is infeasible
		%\State Problem is infeasible
		\Else { $\phi^u$ is  $\epsilon$-global optimal}
		\EndIf
	\end{algorithmic}
	\caption{Variant of Spatial Branch-and-Bound (V-SBB)}% (V-SBB)}%for  problem in \eqref{eq:exactproblem}}
	\label{algo:sbnb}
\end{algorithm}







==> 05-exp.tex <==

We evaluate the performance of our V-SBB algorithm as well as the energy efficiency of our communication, compression and caching (C$3$) joint optimization framework through a series of experiments on several network topologies as shown in Figure~\ref{fig:networks}. {Our key objective is to gain preliminary insights into our algorithm when compared with a few other well-known techniques.} The highlights of the evaluation results are:
\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{networks.pdf}
	\caption{Candidate network topologies used in the experiments: (a) one sink node and one leaf node; (b) one sink node and two leaf nodes; (c) one sink node, one intermediate node and two leaf nodes; and (d) one sink node, two intermediate nodes and four leaf nodes.}
	\protect\label{fig:networks}
	\vspace{-0.1in}
\end{figure}



\begin{itemize}
	\item Our V-SBB algorithm can obtain an $\epsilon$-global optimal solution in most situations within a reasonable time. 
	%the lowest value of the objective function in most situations, i.e., mostly close to the globally optimal solution in reasonable time. 
	Also it is robust and stable to various parameters in different network scenarios. 
	\item When Bonmin \cite{bonami2008algorithmic} can achieve a solution, it is faster. However, the solution obtained through Bonmin is not always comparable to that of V-SBB.  We observe that when higher compression is done (i.e., smaller value of $\gamma$), V-SBB always outperforms Bonmin.  More importantly, we find that Bonmin has poor performance in stability and robustness, i.e., it cannot even produce feasible solutions in some cases although they exist.  NOMAD \cite{le2011algorithm} and GA \cite{deb2002fast} often produce  objective-function values much larger than  V-SBB.
	\item Our C$3$ joint optimization framework improves energy efficiency by as much as $88\%$ compared to the C$2$ optimization over communication and computation, or communication and caching.  
\end{itemize}

\begin{table}[ht]
	%\vspace{-0.1in}
	\centering
	\caption{Characteristics of the solvers used in this paper}
	\vspace{-0.1in}
	\begin{tabular}{|l|p{11.0cm}|}
		%\begin{tabular}{|c|c{6.0cm}|}
		\hline
		\textbf{Solver} & \textbf{Characteristics}  \\ \hline
		\textbf{Bonmin} \cite{bonami2008algorithmic} &  A deterministic approach based on Branch-and-Cut method that solves relaxation problem with Interior Point Optimization tool (IPOPT), as well as mixed integer problem with Coin or Branch and Cut (CBC).  \\ \hline
		%A deterministic  MINLP solver based on branch-and-cut method that solves  the relaxed problem using Interior Point Optimization tool (IPOPT) and uses Coin or Branch and Cut (CBC) for the mixed integer problem                             \\ \hline
		\textbf{NOMAD} \cite{le2011algorithm}  & A stochastic approach based on Mesh Adaptive Direct Search Algorithm (MADS) that guarantees local optimality. It can be used to solve non-convex MINLP and has a relatively good performance.\\ \hline% for derivative free optimization.                      \\ \hline
		\textbf{GA} \cite{deb2002fast} &  A meta-heuristic stochastic approach that can be tuned to solve global optimization problems. We use Matlab \emph{Optimization Toolbox}'s implementation.      \\ \hline
	\end{tabular}
	\vspace{-0.05in}
	\label{tab:Solvercharacteristics}	
\end{table}


\subsection{Methodology}
\noindent{\textbf{\textit{Performance metrics:}}} 
%\begin{comment}
Our primary metrics for comparisons are: \\
\noindent{{\textit{(1) The best solution to the objective function:}}} Since obtaining the global optimum for the NP-hard problem is daunting, we are primarily interested in $\epsilon$-global optimum; \\
%\item Objective Function: The first metric is the ability of the algorithm to obtain a lower value of objective function (as it is a minimization problem). Since obtaining the global optimal is a daunting task, we are primarly interested in $\varepsilon$-global optimality. 
\noindent{{\textit{(2) Convergence Time,}}} which is the time an algorithm needs to obtain the best  solution; \\% The second metric is the time it takes to obtain any solution to the problem. The faster the solution, the better it is. 
\noindent{{\textit{(3) Stability and Robustness,}}} which is characterized by the frequency or ability of the algorithm to  provide  feasible solutions, provided that they are known to exist; \\
\noindent{{\textit{(4) Energy efficiency}}} in joint optimization. We compare the energy cost of our  joint optimization framework for communication, computation and caching (C$3$)  with that of the optimization of any of the two types of resources (denoted by C$2$) under the same situation. The energy efficiency $\mathcal{E}$ defined as:
\begin{align}\label{eq:efficiency}
\mathcal{E}=\frac{E^{\text{total}*}(\text{C}2)-E^{\text{total}*}(\text{C}3)}{E^{\text{total}*}(\text{C}2)}\times 100\%,
\end{align}
where $E^{\text{total}*}(\text{C}3)$ and $E^{\text{total}*}(\text{C}2)$ are the optimal energy costs under the C$3$ optimization framework in~\eqref{eq:optimization} and the C$2$ optimization, respectively.  $\mathcal{E}$ reflects the reduction of energy efficiency for the C$3$ over the C$2$ optimization. 



%percentage of additional cost of C$2$ over C$3$, hence a positive value of $\mathcal{E}$ is preferred, i.e., C$3$ enhances the energy efficiency.  

%In practice, we prefer a highly stable algorithm to achieve an $\epsilon$-global optimal solution in relatively short time. 
%\item Effectiveness: Effectiveness of the algorithm can be defined as the ability of the algorithm to  provide a feasible solution. Effectiveness is one of the more important factors as obtaining a feasible solution is important from practical perspective. 
%\end{enumerate}
%\end{comment}

\begin{table}[ht]
	%\vspace{-0.1in}
	\centering
	\caption{Parameters used in simulations}%Simulation Parameters for Comparing Algorithms}
	%\begin{tabular}{|l|l||l|l|}
	\vspace{-0.1in}
	\begin{tabular}{|c|c||c|c|}
		\hline
		\textbf{Parameter} & \textbf{Value} &\textbf{Parameter} & \textbf{Value (Joules)} \\ \hline
		$y_k$	& 1000 &  $\varepsilon_{vR}$ &  50  $\times$ 10$^{-9}$             \\ \hline
		$R_k$	& 100    & $\varepsilon_{vT}$&   200  $\times$ 10$^{-9}$              \\ \hline
		$w_{ca}$	& 1.88 $\times$ 10$^{-6}$&  $\varepsilon_{cR}$ &  80  $\times$ 10$^{-9}$               \\ \hline
		$T$	& 10s   &$\gamma$ & [$1,\sum_{k \in \mathcal{K}}y_k$]               \\ \hline
	\end{tabular}
	\vspace{-0.1in}
	\label{tab:algcompareparameters}
\end{table}





\noindent{\textbf{\textit{Setup:}}} 
We implement V-SBB in Matlab on a Core i$7$ $3.40$ GHz CPU with $16$ GB RAM.  The candidate MINLP solvers in this work include Bonmin, NOMAD and GA, which are implemented with Opti-Toolbox \cite{optitoolbox}. We summarize the characteristics of these solvers in Table~\ref{tab:Solvercharacteristics}.  Note that these solvers can be applied directly to solve the original optimization problem in \eqref{eq:optimization}, while our V-SBB solves the equivalent problem. % in \eqref{eq:exactproblem}.
The reformulations needed are executed by a Java based module and we derive the bounds on the auxiliary variables. %\blue{given the derived bounds on the auxiliary variables}. 
We also relax the integer constraint in \eqref{eq:optimization} to obtain a non-linear programming problem, which is solved by IPOPT \cite{wachter06} and use it as a benchmark for comparison.  V-SBB terminates when $\epsilon$-optimality is obtained or a computation timer of $200$ seconds expires.  We take $\epsilon=0.001$ in our study.  If the timer expires, the last feasible solution is taken as the best solution.  
%\red{\bf We assume that the transmission cost at sink node is ignore if the data is cached at sink node since our formulation focuses on the cost inside the network.  Thus, once the data is cached at sink node, the energy cost for requesting that data becomes constant since there is no reception and transmission cost.} 
Our simulation parameters are provided in Table~\ref{tab:algcompareparameters}, which  are the typical values used in the literature \cite{nazemi2016qoi, heinzelman2000energy, ye2002energy}.

 \begin{table*}[]
	\centering
	\caption{The Best Solution to the Objective Function (Obj.) and Convergence time for two nodes network}
	\vspace{-0.1in}
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{\textbf{Solver}} & \multicolumn{2}{c|}{{$\gamma=1$}}               & \multicolumn{2}{c|}{{$\gamma= 250$}}      & \multicolumn{2}{c|}{{$\gamma=500$}}     & \multicolumn{2}{c|}{\textbf{$\gamma=750$}}     & \multicolumn{2}{c|}{\textbf{$\gamma=1000$}}    \\ \cline{2-11} 
		& \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s)& \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s) \\ \hline
		\textbf{Bonmin}                  &  0.010&	0.076& 
		0.018&	0.07&	0.026&	0.071&	0.032&	0.077&	0.039&	0.102 \\ \hline
		\textbf{NOMAD}                   & 0.012&	1.036& 
		0.038&	0.739&	0.033&	0.640&	0.038&	0.203&	0.039&	0.263
		\\ \hline
		\textbf{GA}                      & 0.010&	0.286
		&	0.018&	2.817&	0.026&	7.670&	0.042	&11.020	&0.064	&3.330
		\\ \hline
		\textbf{V-SBB}                     & 0.010& 	18.231&
		0.018& 	17.389& 	0.026& 	12.278& 	0.032& 	7.327& 	0.039& 	19.437
		\\ \hline
		\textbf{Relaxed}                 & 0.010&	0.075
		&	0.018&	0.048	&0.026&	0.046&	0.032&	0.050&	0.039&	0.059
		\\ \hline
	\end{tabular}
	\label{tab:results2node}
	\vspace{-0.15in}
\end{table*}






\subsection{The Best Solution to the Objective Function}\label{subsec:value}
 We compare the performance of V-SBB with three other candidate solvers for  the networks in Figure~\ref{fig:networks}.   The results for two nodes and seven nodes networks are presented in Tables~\ref{tab:results2node} and~\ref{tab:results7node}. {We also relax the integer constraint in \eqref{eq:optimization} to be continuous, i.e., $b_{k, i}\in[0, 1]$. Then \eqref{eq:optimization} becomes a geometric programming problem, which can be solved by IPOPT \cite{wachter06}.  We call it ``Relaxed" and the corresponding results are presented in the last row of Tables~\ref{tab:results2node} and~\ref{tab:results7node}. } We observe that V-SBB achieves the lowest value comparable to Bonmin for larger values of $\gamma$, and significantly outperforms Bonmin for smaller values of $\gamma$, which we discuss in detail later.  However, Bonmin cannot generate a feasible solution even if it exists for some cases.  This is because Bonmin is built on the Branch-and-Cut method, which sometimes cuts regions where a lower value exists.  NOMAD and GA in general yield a higher objective-function value than V-SBB does. This is because both NOMAD and GA are based on a stochastic approach which cannot guarantee convergence to the $\epsilon$-global optimum.  Similar trends are observed for three and four node networks, which are presented in Appendix~\ref{sec:appendixg}.
 
 \begin{table*}[]
	\centering
	\caption{The Best Solution to the Objective Function (Obj.) and Convergence time for seven nodes network}
	\vspace{-0.1in}
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{\textbf{Solver}} & \multicolumn{2}{c|}{{$\gamma=1$}}            & \multicolumn{2}{c|}{\textbf{$\gamma=1000$}}      & \multicolumn{2}{c|}{\textbf{$\gamma=2000$}}     & \multicolumn{2}{c|}{\textbf{$\gamma=3000$}}     & \multicolumn{2}{c|}{\textbf{$\gamma=4000$}}    \\ \cline{2-11} 
		& \textbf{Obj.} & \textbf{Time} (s) &  \textbf{Obj.} &\textbf {Time} (s) & \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s) \\ \hline
		\textbf{Bonmin}                  & 0.0002&	0.214
		&	0.039&	0.164&	0.078&	0.593&	0.117&	0.167&	0.156	&0.212
		
		\\ \hline
		\textbf{NOMAD}                   & 0.004&	433.988& 
		0.121&	381.293&	0.108&	203.696&	0.158&	61.093&	0.181&	26.031
		\\ \hline
		\textbf{GA}                      & 0.043&	44.538	
		&0.096	&30.605	&0.164	&44.970	&0.226&	17.307	&0.303	&28.820
		\\ \hline
		\textbf{V-SBB}                     & 0.0001& 	1871.403&
		0.039& 	25.101& 	0.078& 	30.425& 	0.117& 	23.706& 	0.156	& 19.125
		\\ \hline
		\textbf{Relaxed}                 & 0.0002	&0.201
		&	0.039	&0.111	&0.078	&0.095&	0.117&	0.102&	0.156&	0.105
		\\ \hline
	\end{tabular}
	\label{tab:results7node}
	\vspace{-0.15in}
\end{table*}


\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{R-monotone}
	\caption{Total Energy Costs vs. Number of Requests.}% paradigms.}
	%\caption{Monotonicity of the total energy consumption with increase in number of Requests}
	\label{fig:mono2node}
	\vspace{-0.2in}
\end{figure} 

Figure~\ref{fig:mono2node} verifies that the optimal energy cost is monotonically increasing with the number of requests, as stated in Remark~\ref{thm:increasingR} for a two node and seven node network. The results are obtained using our C3 framework for $\gamma=0.25\sum_{k \in \mathcal{K}}y_k$ and $\gamma=0.75\sum_{k \in \mathcal{K}}y_k,$ respectively. For the network parameters under consideration, we note that there is a turning point on the curves, and the total energy cost increases much faster with the number of requests before the turning point than that after it.   This is because the data has already been cached at the root node at this point and there is no need to retrieve data from other nodes in the network, which reduces transmission costs.  This is the benefit that caching brings, and we will further discuss the advantage of C$3$ optimization over the C$2$ later in Section~\ref{subsec:efficiency}. 




\subsection{Convergence Time}\label{subsec:speed}
The time taken to obtain the best solution is important in practice.  The amount of time that an algorithm requires to obtain its best solution as discussed in Section~\ref{subsec:value}  are shown in Tables~\ref{tab:results2node} and~\ref{tab:results7node} for the two nodes and seven nodes networks, respectively.  It  can be see that Bonmin is the fastest method since it uses the branch-and-cut approach which cuts certain domains to accelerate the branching process.  As discussed earlier, the Bonmin algorithm is fast at the expense of algorithm stability, i.e., sometimes it cannot find a solution although it exists.  This will be further discussed in the following section.  V-SBB takes longer to obtain a better solution, because our reformulation introduces auxiliary variables and additional linear constraints.   Different applications can tolerate various degrees of algorithm speed. For the sample networks and applications under consideration, the speed of V-SBB is considered to be acceptable \cite{floudas2013deterministic}. 



\subsection{Stability}\label{subsec:stability}
From the analysis in Sections~\ref{subsec:value} and~\ref{subsec:speed}, we know that Bonmin is faster but unstable in some situations.  We further characterize the stability of Bonmin with respect to the threshold value of QoI $\gamma$ as follows. Specifically, we fix all other parameters  in Table~\ref{tab:algcompareparameters}, and vary only the maximal possible value of $\gamma$ in different networks. The results are shown in Table~\ref{tab:bonmininfeas}. For each maximal value, we test all the possible integer values of $\gamma$ between $1$ and itself. Hence, the number of tests equals the maximal value.  We see that the number of instances where the Bonmin method fails to produce a feasible solution increases as the network size increases.  This is mainly due to the cutting phase in the Bonmin method, which cuts the feasible regions that need to be branched. 

\begin{table}
	%\vspace{-0.1in}
	\centering
	\caption{Infeasibility of Bonmin for networks in Figure~\ref{fig:networks}}
	\vspace{-0.1in}
	%\begin{tabular}{|l|l|l|l|l|}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\textbf{Networks}  & (a) &  (b) &  (c) &  (d) \\ \hline
		\textbf{$\#$ of test values}      & {1000} & {2000} & {2000} & 4000 \\ \hline
		\textbf{$\#$ of infeasible solutions} & 0              & 0            & 1            & 216          \\ \hline
		\textbf{Infeasibility (\%)} & 0              & 0           & 0.05           & 5.4          \\ \hline
	\end{tabular}
	\vspace{-0.2in}
	\label{tab:bonmininfeas}
\end{table}


\begin{table*}[ht]
	\centering
	\caption{Comparison between V-SBB and Bonmin for smaller values of $\gamma$ in seven node network}
	\vspace{-0.1in}
	\label{tab:improvement}
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{\textbf{Solver}} & \multicolumn{2}{c|}{$\gamma$ =1} & \multicolumn{2}{c|}{$\gamma$=3} & \multicolumn{2}{c|}{$\gamma$ =5} & \multicolumn{2}{c|}{$\gamma$ =8} & \multicolumn{2}{c|}{$\gamma$ =50} \\ \cline{2-11} 
		& \textbf{Obj.}   & \textbf{Time (s)}  & \textbf{Obj.}    & \textbf{Time}    & \textbf{Obj.}     & \textbf{Time}    & \textbf{Obj.}     & \textbf{Time}    & \textbf{Obj.}     & \textbf{Time}     \\ \hline
		\textbf{Bonmin}                  & 0.0002 &	0.214 &	0.0003 &	0.211 &	0.0003 &	0.224 &	 0.0005&	0.23&	0.0021&	0.364
		\\ \hline
		\textbf{V-SBB}                   & 0.00011&	1871.403&	0.00015&	2330&	0.00019&	1243.77	&0.00047	&1350.016&	0.0020	&3325.302
		\\ \hline
		\textbf{Improvement (\%)}             & \multicolumn{2}{c|}{52.45}           & \multicolumn{2}{c|}{49.43}          & \multicolumn{2}{c|}{50.30}          & \multicolumn{2}{c|}{7.59}         & \multicolumn{2}{c|}{4.62}   \\ \hline
	\end{tabular}
	\vspace{-0.1in}
\end{table*}

Although Bonmin can provide a feasible solution for smaller values of $\gamma$ at a faster time, we observe that the value of the solution is larger than that of V-SBB.  We compare the performance of V-SBB and Bonmin for smaller values of $\gamma$ in Table~\ref{tab:improvement}.  We see that V-SBB outperforms Bonmin by as much as $52.45\%$ when searching for an $\epsilon$-global optimum, though it requires more time. The timer is set to $7200$s for results shown in Table~\ref{tab:improvement}. 
%\red{With the increase in the number of nodes, Bonmin's performance deteriorates and it converges to an infeasible point. Even when Bonmin provides feasible solution for lower values of $\gamma$, the value of the solution is higher than the ones obtained with V-SBB. Table \ref{tab:improvement} compares the performance of V-SBB with Bonmin and shows that V-SBB outperforms Bonmin by as much as 52.45\% when searching for an $\epsilon-$global optimal; however it requires more time. }



% Please add the following required packages to your document preamble:
% \usepackage{multirow}

%\subsection{Advantage of using joint communication, computation and caching} 
\subsection{Energy Efficiency} \label{subsec:efficiency}
We compare the total energy costs under joint C$3$ optimization with those under C$2$ optimization. We consider two cases for the C$2$ optimization: (i) C$2$o (Communication and Computation), where we set $S_v=0$ for each node to avoid any data caching; (ii) C$2$a (Communication and Caching), where we set $\gamma=\sum_{k \in \mathcal{K}}y_k,$ which is equivalent to $\delta_v=1,$ $\forall v\in V$, i.e., no computation. Comparison between C$3$, C$2$o and C$2$a is shown in Figure~\ref{fig:c3vsc2}.  

\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{c3vc2}
	\caption{Comparison of C$3$ and C$2$ optimization for the seven node network in Figure~\ref{fig:networks}.}% in terms of objective function and different number of Requests for a 2-node network}
	\label{fig:c3vsc2}
	\vspace{-0.2in}
\end{figure} 

First, we observe that as the number of requests increases, the total energy cost increases, as reflected in Remark~\ref{thm:increasingR}.  Second,  the energy cost for the C$3$ joint optimization is lower than that for  C$2$o optimization for the same parameter setting.  This captures the tradeoff between caching, communication and computation.  In other words, although C$3$ incurs caching costs, it may significantly reduce the communication and computation, which in turn brings down total energy cost.   Similarly, C$3$ optimization outperforms C$2$a although C$3$ incurs caching cost.  Using Equation~(\ref{eq:efficiency}), energy efficiency improves by as much as $88\%$ for the C$3$ framework when compared with the C$2$ formulation.  These trends are observed  in other candidate network topologies. Details for the 2 node network can be found in Appendix~\ref{sec:appendixf}. 
\begin{rem}
	Note that the above results are based on parameter values typically used in the literature, as shown in Table~\ref{tab:algcompareparameters}. From our analysis, it is clear that the larger the ratio between $\varepsilon_{vT}$ and $\varepsilon_{vR}$, $\varepsilon_{vC}$, the larger will be the improvement provided by our C$3$ formulation.
\end{rem}







==> 05-related.tex <==



A key focus of this work is to demonstrate and validate the joint application of data computation and caching, specifically in geo-distributed systems, e.g., WSNs, to achieve minimal energy consumption due to data communication, computation and caching with a QoI guarantee.  Key decisions for a geo-distributed system are how much of the computation should be performed at each server and where the data should be cached in the system.  The basic building blocks of our model {are} simple and have been studied in various settings.  However, to the best of our knowledge,   there is no prior work that jointly considers communication, computation and caching costs in data communication networks with a QoI guarantee for end users. %One of the important contributions of this paper is to develop an optimization algorithm that minimizes the total system energy costs by characterizing the tradeoff between communication, computation and caching costs with a QoI guarantee for end users. 



\noindent{\textit{\textbf{Data Compression:}}} Compression is a key operator in data analytics and has been supported by many data-parallel programming models \cite{boykin14}.  For WSNs, data compression is usually performed over a hierarchical topology to improve communication energy efficiency \cite{rajagopalan06}, whereas we focus on energy tradeoff between communication, computation and caching. 

\noindent{\textit{\textbf{Data Caching:}}}  Caches play a significant role in many systems with hierarchical topologies, e.g., WSNs, microprocessors, CDNs etc.  There is a rich literature on the performance of caching in terms of designing different caching algorithms, e.g., \cite{garetto16, fofack12,jian17,ioannidis16}, and we do not attempt to provide an overview here.  Utility maximization approach has also been studied for cache management \cite{dehghan16,nitishjian17,nitishjianfaheem17}.  However, none of these work considered the costs of caching, which may be significant in some systems \cite{choi2012network}.% \red{Dimokas et al. \cite{dimokas2008cooperative} presented a cooperative caching protocol designed for WSNs. Dimokas et al. \cite{dimokas2011high} also proposed two cooperative caching protocols for WSNs that minimized latency and improved the energy efficiency of the WSN.  Alipio et al. \cite{alipio2017cache} presented a detailed survey on cache based transport protocols for WSNs. } \blue{[\bf{not sure if this is the right position. May motivate it in the introduction. I will do that. }]}


\noindent{\textit{\textbf{Energy Costs:}}}  While optimizing energy costs in wireless sensor networks has been extensively studied \cite{heinzelman2000energy,ye2002energy}, existing work primarily is concerned with routing \cite{manjeshwar2001teen}, MAC protocols \cite{heinzelman2000energy}, and clustering \cite{ye2005eecs}. With the growing deployment of smart sensors in modern systems \cite{nazemi2016qoi}, in-network data processing, such as data aggregation, has been widely used as a mean of reducing system energy cost by lowering the data volume for transmission. 

Energy efficient inference in a random fusion network without QoI guarantee was considered in \cite{anandkumar2009energy}.  Network Utility Maximization (NUM) framework was applied in \cite{laporta2012} to obtain optimal compression rate for data aggregation as well as optimal locations for performing data compression.   The optimal energy allocation between communication and sensing to maximize the total information received at the sink node was studied in \cite{zhang2006distributed}, but they did not consider data computation.  An efficient algorithm for data compression in a  data gathering tree was proposed in \cite{yu2008data}.   A distributed algorithm to minimize overall energy costs in a tree structured network by optimizing the compression factor at  each node was presented in \cite{nazemi2016qoi}.  While these work only focus on energy costs of data communication and compression, we study the energy tradeoff between data communication, computation and caching. 

%None of these works considered caching costs.  Since caches are already integral components of many modern systems, including wireless sensor networks, they can be used to improve performance by making data available at locations closer to end users to reduce the communication cost \cite{choi2012network}.



%To the best of our knowledge, there is no prior work that jointly considers communication, computation and caching costs in data communication networks. One of the important contributions of this paper is to develop an optimization algorithm that minimizes the total system energy costs by characterizing the tradeoff between communication, computation and caching costs with a QoI guarantee for end users. 

==> 12-appF.tex <==
%\newpage
Figure \ref{fig:c3vsc2-2node} shows the improvement  that C$3$ brings in comparison with C$2$ for a two nodes network. Using Equation~(\ref{eq:efficiency}), energy efficiency improves by as much as $70\%$ for the C$3$ framework when compared with the C$2$ formulation.
\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{c3vc2-2node}
	\captionsetup{justification=centering}
	\caption{Comparison of C$3$ and C$2$ optimization for the two nodes network in Figure~\ref{fig:networks}.}% in terms of objective function and different number of Requests for a 2-node network}
	\label{fig:c3vsc2-2node}
	%\vspace{-0.2in}
\end{figure} 


%\newpage

==> 13-appG.tex <==
The results for three nodes and four nodes networks are presented in Tables~\ref{tab:results3node} and~\ref{tab:results4node}. 
\begin{table}
	\centering
	\caption{The Value of Objective Function (Obj.) and Convergence Speed for three node network}
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{\textbf{Solver}} & \multicolumn{2}{c|}{{$\gamma=1$}}               & \multicolumn{2}{c|}{{$\gamma= 5000$}}      & \multicolumn{2}{c|}{{$\gamma=10000$}}     & \multicolumn{2}{c|}{\textbf{$\gamma=15000$}}     & \multicolumn{2}{c|}{\textbf{$\gamma=20000$}}    \\ \cline{2-11} 
		& \textbf{Obj.} & \textbf{Time} (s) 	& \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s)& \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s) \\ \hline
		\textbf{Bonmin}                  & 0.005&	0.321&
		0.010&	0.104&	0.019&	0.091&	0.029&	0.093&	0.038&	0.101
		
		\\ \hline
		\textbf{NOMAD}                   & 0.045&	11.254&
		0.025&	9.407&	0.033&	8.739&	0.030&	40.517&	0.038&	4.038
		
		\\ \hline
		\textbf{GA}                      & 0.025&	0.509&		0.010&	9.799&	0.027&	4.924&	0.045&	19.045&	0.050	&2.154
		
		\\ \hline
		\textbf{Our}                     & 0.005&	200	&
		0.010&	200&0.020&	200&	0.029&	200&	0.038&	1.223
		
		\\ \hline
		\textbf{Relaxed}                 &0.005&	0.060&
		0.010&	0.056&	0.019&	0.058&	0.029&	0.050&	0.038&	0.048
		
		\\ \hline
	\end{tabular}
	\label{tab:results3node}
\end{table}


\begin{table}
	\centering
	\caption{The Value of Objective Function (Obj.) and Convergence Speed for four node network}
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{\textbf{Solver}} & \multicolumn{2}{c|}{{$\gamma=1$}}              & \multicolumn{2}{c|}{{$\gamma= 5000$}}      & \multicolumn{2}{c|}{{$\gamma=10000$}}     & \multicolumn{2}{c|}{\textbf{$\gamma=15000$}}     & \multicolumn{2}{c|}{\textbf{$\gamma=20000$}}    \\ \cline{2-11} 
		& \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} &  \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s)& \textbf{Obj.} & \textbf{Time} (s) & \textbf{Obj.} & \textbf{Time} (s) \\ \hline
		\textbf{Bonmin}                  &0.002&	0.337&
		0.020	&0.104&	0.040&	0.104&	0.059&	0.100&	0.079&	0.139
		
		\\ \hline
		\textbf{NOMAD}                   & 0.003&	101.891	&
		0.023&	90.626&	0.040&	52.293&	0.060&	47.068&	0.104&	2.070
		
		\\ \hline
		\textbf{GA}                      & 0.002&	0.692&
		0.020&	25.615&	0.042&	7.84&	0.107&	23.770&	0.104&	6.636
		
		\\ \hline
		\textbf{Our}                     & 0.002&	200&
		0.020&	200	&0.052&	200&	0.059&	200	&0.079&	13.344
		
		\\ \hline
		\textbf{Relaxed}                 & 0.002&	0.500&
		0.020&	0.066&	0.040&	0.062&	0.059&	0.073&	0.079&	0.083
		\\ \hline
	\end{tabular}
	\label{tab:results4node}
\end{table}


